HardCoRe-NAS: Hard Constrained diffeRentiable Neural Architecture Search

Realistic use of neural networks often requires adhering to multiple constraints on latency, energy and memory among others. A popular approach to find fitting networks is through constrained Neural Architecture Search (NAS), however, previous methods enforce the constraint only softly. Therefore, the resulting networks do not exactly adhere to the resource constraint and their accuracy is harmed. In this work we resolve this by introducing Hard Constrained diffeRentiable NAS (HardCoRe-NAS), that is based on an accurate formulation of the expected resource requirement and a scalable search method that satisfies the hard constraint throughout the search. Our experiments show that HardCoRe-NAS generates state-of-the-art architectures, surpassing other NAS methods, while strictly satisfying the hard resource constraints without any tuning required.

==> abstract-old.tex <==
\begin{abstract}
 Realistic use of neural networks often requires adhering to multiple constraints on, for example, performance, latency, energy and memory. 
A popular approach to find fitting networks is through constrained Neural Architecture Search (NAS), however, previous methods enforce the constraint only softly. 
%This is done either by prediction of the resources on some validation set, which is inaccurate by nature, or by optimizing an objective that balances accuracy and a soft penalty on the resources, which, tends to be sensitive to the tuning of the trade-off. 
Therefore,  the resulting networks do not exactly adhere to the resource constraint and their accuracy is harmed.
In this work we resolve this by introducing \textit{Hard Constrained diffeRentiable NAS (HardCoRe-NAS)}, that is based on accurate (hard) formulation of the expected resource requirement, and a search method that satisfies the constraint throughout the optimization.
Our experiments show that HardCoRE-NAS converges faster than other gradient-based methods, while at the same time generating architectures with higher accuracy that strictly satisfy the resource constraint. 
 
 
\end{abstract}

% Neural Architecture Search (NAS) has been of broad interest in recent years, aiming for an automatic design of optimized neural architectures for given tasks. Practical considerations invite the search for maximal accuracy under latency/energy/memory requirements on a target device. Previous approaches address those requirements by adding a penalty term to the loss resulting a trade-off between accuracy and resources. This penalty hardens the optimization process, which is much sensitive to the tuning of such trade-offs and thus the exact satisfaction of the resource budget is oftentimes missing.
% We introduce Hard Constrained Differentiable NAS (HCD-NAS) for alleviating those challenges.
% For this purpose we construct a search space capable of parameterizing neural structures with different operations, width and depth in a fully differentiable manner. We further suggest an accurate formula for the expected latency of every architecture residing in that space. Finally we search in the space by solving a constrained optimization problem using the block coordinate stochastic Frank-Wolfe (BC-SFW) algorithm while tightly satisfying the expected latency constraint anytime along the search. Thus soft penalties and the associated trade-offs are mitigated.
%  We show empirical results of 78.3/77.2/75.7\% top-1 accuracy on ImageNet running at 61/48/39ms on an Intel Xeon CPU respectively, surpassing state-of-the-art models both designed manually and generated automatically, while HCD-NAS converges faster than other gradient-based methods, and generates architectures that strictly satisfy the latency constraint.
 

==> big_table_v0.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{|l|c|c||c|c||c|}
    \hline 
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{CPU} & \multicolumn{2}{c}{GPU} &  \multirow{2}{*}{\makecell[l]{Search + Training \\ Cost (GPU hours)}}\\ 
     & Latency (ms) & Accuracy (\%) & Latency (ms) & Accuracy (\%) &
    \\\hline \hline
         MobileNetV2 & 70 & 76.5 & 50 & 76.5 & 150N \\ \hline 
         MobileNetV3 & 45 & 75.2 & 28 & 75.2 & 180N \\ \hline
         EfficientNet B0& 85 & 77.3 & 48 & 77.3 & ? \\ \hline 
         TF-NAS-A & 40 & 74.4 & 54 & 76.9 & \multirow{4}{*}{263N} \\ \cline{1-5}
         TF-NAS-B & 60 & 75.8 & 44 & 76.3 & \\ \cline{1-5}
         TF-NAS-C & & & 37 & 75.2 & \\ \cline{1-5}
         TF-NAS-D & & & 30 & 74.2 & \\ \hline
        %  MNAS-NET & 36 & 74.5 \\ \hline
         MNAS-NET A1 & 55 & 75.2 & 37 & 75.2 & \multirow{2}{*}{40,000N} \\ \cline{1-5}
         MNAS-NET B1 & 39 & 74.5 & 34 & 74.5 & \\ \hline
         FB-NET & 47 & 75.1 & 41 & 75.1 & 576N \\ \hline
         SP-NASNET & 41 & 74.1 & 36 & 74.1 & 288 + 408N\\ \hline
         OFA & 42 & 75.7 & & & 1200 + 25N \\ \hline \hline
         \textbf{Ours 25 ms} & & & 27 & 75.7 & \multirow{8}{*}{400 + 78N}\\ \cline{1-5} 
         \textbf{Ours 30 ms} &  & & 32 & 76.5 & \\ \cline{1-5} 
         \textbf{Ours 40 ms} & 40 & 75.8 & 41 & 77.5 & \\ \cline{1-5} 
         \textbf{Ours 45 ms} & 44 & 76.4 & & & \\         \cline{1-5} 
         \textbf{Ours 50 ms} & 50 & 77.1 & & & \\ \cline{1-5}
         \textbf{Ours 55 ms} & 55 & 77.6 & & & \\ \cline{1-5}
         \textbf{Ours 60 ms} & 61 & 78.0 & & & \\ \hline
    \end{tabular}
    \caption{ImageNet top-1 accuracy and search time comparison with other methods. Latency is reported for Intel Xeon CPU and NVIDIA P100 GPU with a batch size of 1 and 64 respectively}
    \label{tab:exp_cpu}
\end{table*}



% \begin{table}[t]
%     \centering
%     \begin{tabular}{|l|c|c|}
%     \hline 
%     Model & latency (ms) & accuracy (\%) \\ \hline
%          MobileNet v3 & 45 & 75.2 \\ \hline
%          EfficientNet B0& 85 & 77.3 \\ \hline 
%          TF-NAS-CPU A & 40 & 74.4 \\ \hline
%          TF-NAS-CPU B & 60 & 75.8 \\ \hline
%         %  MNAS-NET & 36 & 74.5 \\ \hline
%          MNAS-NET A1 & 55 & 75.2 \\ \hline
%          MNAS-NET B1 & 39 & 74.5 \\ \hline
%          FB-NET & 47 & 75.1 \\ \hline
%          SP-NASNET & 41 & 74.1 \\ \hline
%          MobileNet v2 (x140) & 70 & 76.5 \\ \hline
%          OFA-CPU & 42 & 75.7 \\ \hline
%          \hline
%          \multicolumn{3}{|l|}{Training from scratch} \\ \hline
%          \textbf{Ours 40 ms} & 40 & 75.8 \\ \hline
%          \textbf{Ours 45 ms} & 44 & 76.4 \\ \hline
%          \textbf{Ours 50 ms} & 50 & 77.1 \\ \hline
%          \textbf{Ours 55 ms} & 55 & 77.6 \\ \hline
%          \textbf{Ours 60 ms} & 61 & 78.0 \\ \hline
%         %  \multicolumn{3}{|l|}{OFA pretraining, 25 epochs fine-tune} \\ \hline
%         %  \textbf{Ours 40 ms} & 39 & 75.7 \\ \hline
%         %  \textbf{Ours 45 ms} & 45 & 76.7 \\ \hline
%         %  \textbf{Ours 50 ms} & 49 & 77.2 \\ \hline
%         %  \textbf{Ours 55 ms} & 56 & 77.9 \\ \hline
%         %  \textbf{Ours 60 ms} & 60 & 78.3 \\ \hline
%         %  \hline
%     \end{tabular}
%     \caption{Imagenet Accuracy vs Latency on Intel Xeon CPU for a batch size of 1}
%     \label{tab:exp_cpu}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|l|c|c|}
%     \hline 
%     Model & latency (ms) & accuracy (\%) \\ \hline
%          MobileNet v3 & 28 & 75.2 \\ \hline
%          TF-NAS-GPU D & 30 & 74.2 \\ \hline
%          \textbf{Ours 25 ms} & \textbf{27} & \textbf{75.7} \\ \hline \hline
%          MNAS-NET B1 & 34 & 74.5 \\ \hline
%          SP-NASNET & 36 & 74.1 \\ \hline
%          TF-NAS-GPU B & 44 & 76.3 \\ \hline
%          TF-NAS-GPU C & 37 & 75.2 \\ \hline
%          MNAS-NET A1 & 37 & 75.2 \\ \hline
%          FB-NET & 41 & 75.1 \\ \hline
%          \textbf{Ours 30 ms} & \textbf{32} & \textbf{76.5} \\ \hline \hline
%          TF-NAS-GPU A & 54 & 76.9 \\ \hline
%          EfficientNet B0& 48 & 77.3 \\ \hline 
%          MobileNet v2 (x140) & 50 & 76.5 \\ \hline
%          \textbf{Ours 40 ms} & \textbf{41} & \textbf{77.5} \\ \hline
%     \end{tabular}
%     \caption{Imagenet Accuracy vs Latency on NVIDIA P100 GPU for a batch size of 64}
%     \label{tab:exp_GPU}
% \end{table}

==> exp_v0.tex <==
\section{Experimental Results}\label{sec:experiments}
\subsection{Validation of the Latency Formula}\label{sec:validate_latency}
Aiming at providing a practical method to accurately fit the user's resource requirements, we validate the accuracy of our latency formula (\ref{eqn:latency_formula}) by comparing its outcome to the measured latency for several models on Intel Xeon CPU and NVIDIA P100 GPU. The measurements are shown in Figure~\ref{fig:latency}, admitting a linear relation with the ratio of $1.003$ and a coefficient of determination of $R^2=0.99$. This validates the accuracy of the proposed formula.

\subsection{Evaluating the Solution of the Inner Problem $w^*$}\label{sec:evaluate_inner}
The ultimate quality measure for a generated architecture is arguably its accuracy over a test set when trained as a stand-alone model from randomly initialized weights.
Hence, relaying on the solution $w^*$ of the inner problem of (\ref{eqn:NAS_bilevel}) for searching the space (section \ref{sec:outer_problem}) requires the one-shot model equipped with $w*$ to admit correlated rankings of the accuracy of sub-netwroks extracted from it and their corresponding stand-alone accuracy.
For the evaluation of this correlation, we calculate the Kendall-Tau \cite{KendallTau} and Spearman's \cite{spearman1961general} rank correlation coefficients, denoted as $\tau$ and $\rho$ respectively.
To this end extract 18 sub-networks over the entire search space $d\in \{2,3,4\}$ expansion ratio $er\in\{3,4,6\}$ and kernel $k\in\{3,5\}$, train them from scratch for 200 epochs, and extract their final accuracy. Next, we compare three pretraining methods: Our pretraining involving 250 epochs of training the highest possible network, intitializing the super-network with these weights and fine-tuning it for 100 epochs using the multi-path sampling method, and two simple pretrainings of the network where the entire super-network is trained from scratch for 100 epochs, with and without multipath sampling method. We compare the accuracy of the extracted corresponding 18 networks from the different pretrained super-networks with the accuracy we got from training these networks from scratch, by computing the Kendal-Tau and Spearman metrics between them.  Since our method relay on the gradient of the loss with respect to the architectures parameters, it is important to have a pretraining that can rank the network correctly. In figure (\ref{fig:acc_kendal_tau}), we compare the accuracy of architecture extracted from our super-network with the robust pretraining and a simple pretraining against the accuracy of the same network trained from scratch. As we can see, using a more robust pretraining allows for the extracted architecture to have an accuracy (and hence a loss) that is much more correlated to the true accuracy of the extracted network. 
We compare the Kendall-Tau ($\tau$) and Spearman ($\rho$) correlations  between the accuracy of the networks extracted from the three pretrained super-networks (advanced and simple with and without multipath) and the accuracy of these networks from scratch. For a robust pretraining, the metric are $\tau=0.95, \rho=0.99$ while the latter for a simple multipath pretraining are $\tau=0.84, \rho=0.95$, and $\tau=0.35, \rho=0.44$ for a single-path simple pretraining. We can conclude that both our pretraining and sampling strategy allows to get a super-network whose accuracy of every extracted sub-network is strongly correlated to its accuracy from scratch. This observation justifies the fact that we do not update the weights of the super-network during the search.


% \subsection{Comparison with soft penalty}
% Todo: Add graphs where we see a jitter around the target latency when using TF-NAS penalty

\subsection{Outer Problem: Hard vs Soft Constraint}
\subsubsection{Toy Problem}
\label{subsec:toy_example}
In order to motivate the need for expressing the NAS problem using BCFW algorithm, we present a toy example based on quadratic programming. Our purpose is to solve the following optimization problem:
\begin{equation}
    \label{eqn:toy_ex}
    \begin{array}{l}
       \min_x \|x\|^2 \\
       \text{s.t}\\
       \sum_i x_i = 1
    \end{array}
\end{equation}
To this end, we can either use FW algorithm, or Gradient Descent (GD) with a hard penalty constraint, i.e. minimizing $\|x\|^2+\lambda \left(\sum_i x_i - 1\right)^2$ when $\lambda$ is a coefficient controlling the penalty. We use a dimensionality of $10$ for our problem, meaning that $x\in\mathbb{R}^{10}$. The solution of the problem can be computed analytically, and consists in a uniform vector whose all entries are $\frac{1}{d}$ where $d$, the dimension of the problem is 10 in our case, such as the optimal objective loss is $0.1$. In order to start with a feasible solution, we simply draw a random vector from uniform distribution and normalize its entries by dividing it by the sum of its components. One of the difficulties of using penalty loss is to tune the penalty coefficient $\gamma$, that represents the compromise between the minimization of the objective function and the respect of the constraint. In figure \ref{fig:fw_vs_gd}, we compare both objective and constraint losses for FW and GD with penalty algorithms. We can see that not only FW converges faster while respecting the constraint at every step of the optimization, it does not require to tune for an additional $\lambda$ parameter. When using GD with penalty, either the loss converges fast but not respecting the constraint (blue entries for $\lambda=1$) or the constraint is almost respected, but the convergences to the minimum is much slower than the FW one. In addition we can see that the constraint loss when using GD with hard penalty is never zero, even for higher values of $\lambda$.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/gd_diff_lambda.pdf}
    \caption{Objective loss and constraint loss of FW and hard penalty constraint GD for different values of hard penalty constraint $\lambda$. Continuous entries represent the objective loss (left y-axis) while dashed entries represent the constraint loss (right y-axis)}
    \label{fig:fw_vs_gd}
\end{figure}
\subsubsection{Ablation Study}

\subsection{Dataset and setting}
We apply our search method on the ImageNet Dataset, selecting $20\%$ of the training set as validation set. Our target device is a Intel XEON CPU, and we search for architectures with latencies $40, 45, 50, 55$ and $60$ milliseconds. For all of our experiments, we train our networks with SGD using label smoothing 0.1; mixup 0.2; Autoaugment; learning rate $0.1$; weight decay $10^{-4}$; and Nesterov momentum of $0.9$. We perform pretraining or our elastic network by first training the highest network (depth 4, expansion ratio 6, kernel 5) for 250 epochs and then fine-tuning the entire elastic network with 100 epochs. Unlike OFA that requires $250+3\times 120$ epochs, our procedure of pretraining requires only 350 epochs, since it is the ranking between the different sub-networks that matters rather than their final accuracy.
After our elastic network is pretrained, we apply our search method on a validation set composed by $20\%$ of the training set, and the search time is few GPU hours, since it requires only 6 epochs on the validation set, that is the equivalent in term of computational cost of a single epoch on the all training set.
\subsection{Comparisons with Current SOTA}
We test our method on Intel XEON CPU. For every of the networks we are comparing to, we take its official Pytorch implementation and measure the latency using a single thread without optimization such as MKL-DNN, in the exact same condition as for our networks. For this reason, the latency we report may differ from the latency reported in other papers, that may use optimization engine such as MKL-DNN or OpenVino. In order to have a fair comparison with methods not using robust pretraining, after an architecture is found, we train it from scratch in order to reflect the potential of our found architecture rather that the advantage of using a robust pretraining. We present our results in table \ref{tab:exp_cpu} and figure \ref{fig:acc_nas}. We can see that the latency of every found network corresponds to its target, and that the accuracy of the corresponding networks trained from scratch surpasses every other cited methods. In addition, in the second part of the table \ref{tab:exp_cpu} we present results with a pretraining that has followed the OFA progressive shrinking scheme, and with a fine tuning of 25 epochs after the architecture is found. As can be seen in table \ref{tab:exp_cpu}, our found network for $40$ ms latency reaches $74.8\%$ accuracy on ImageNet, that is $0.4\%$ better than TF-NAS-CPU-A \cite{TF-NAS}, $0.7\%$ better than SP-NASNET \cite{SPNAS} with similar or higher latency, while our $50$ ms latency network reaches $76.0\%$ accuracy, that is $0.9\%$ better than FB-NET \cite{fbnet}, $0.8\%$ better than MobileNetV3 \cite{mobilenetv3} and $0.3\%$ better than OFA \cite{OFA} with similar or higher latency. Our $55$ ms network reaches $76.9\%$ accuracy, that is $1.7\%$ higher that MNASNET-A1 \cite{tan2019mnasnet} whose search requires more than 90.000 GPU hours. Finally, our $60$ latency networks reaches $77.1\%$ accuracy, that is $1.3\%$ better than TF-NAS-CPU-B with similar latency, $0.6\%$ accuracy higher than MobileNet V2 \cite{mobilenetv2}, while being $10$ ms faster,  and just $0.2\%$ worse than EfficientNet B0 \cite{effnet} while being $25$ ms faster. 
In addition, in table \ref{tab:exp_GPU}, we also compare out method with others on NVIDIA P100 GPU.
\begin{table}[t]
    \centering
    \begin{tabular}{|l|c|c|}
    \hline 
    Model & latency (ms) & accuracy (\%) \\ \hline
         MobileNet v3 & 45 & 75.2 \\ \hline
         EfficientNet B0& 85 & 77.3 \\ \hline 
         TF-NAS-CPU A & 40 & 74.4 \\ \hline
         TF-NAS-CPU B & 60 & 75.8 \\ \hline
        %  MNAS-NET & 36 & 74.5 \\ \hline
         MNAS-NET A1 & 55 & 75.2 \\ \hline
         MNAS-NET B1 & 39 & 74.5 \\ \hline
         FB-NET & 47 & 75.1 \\ \hline
         SP-NASNET & 41 & 74.1 \\ \hline
         MobileNet v2 (x140) & 70 & 76.5 \\ \hline
         OFA & 42 & 75.7 \\ \hline
         \hline
         \multicolumn{3}{|l|}{Training from scratch} \\ \hline
         \textbf{Ours 40 ms} & 40 & 75.8 \\ \hline
         \textbf{Ours 45 ms} & 44 & 76.3 \\ \hline
         \textbf{Ours 50 ms} & 50 & 76.8 \\ \hline
         \textbf{Ours 55 ms} & 55 & 76.9 \\ \hline
         \textbf{Ours 60 ms} & 61 & 77.1\\ \hline
         \multicolumn{3}{|l|}{OFA pretraining, 25 epochs fine-tune} \\ \hline
         \textbf{Ours 40 ms} & 39 & 75.7 \\ \hline
         \textbf{Ours 45 ms} & 45 & 76.7 \\ \hline
         \textbf{Ours 50 ms} & 49 & 77.2 \\ \hline
         \textbf{Ours 55 ms} & 56 & 77.9 \\ \hline
         \textbf{Ours 60 ms} & 60 & 78.3 \\ \hline
         \hline
    \end{tabular}
    \caption{Imagenet Accuracy vs Latency on Intel Xeon CPU for a batch size of 1}
    \label{tab:exp_cpu}
\end{table}


\begin{table}[t]
    \centering
    \begin{tabular}{|l|c|c|}
    \hline 
    Model & latency (ms) & accuracy (\%) \\ \hline
         MobileNet v3 & 28 & 75.2 \\ \hline
         TF-NAS-GPU D & 30 & 74.2 \\ \hline
         \textbf{Ours 25 ms} & \textbf{27} & \textbf{75.7} \\ \hline \hline
         MNAS-NET B1 & 34 & 74.5 \\ \hline
         SP-NASNET & 36 & 74.1 \\ \hline
         TF-NAS-GPU B & 44 & 76.3 \\ \hline
         TF-NAS-GPU C & 37 & 75.2 \\ \hline
         MNAS-NET A1 & 37 & 75.2 \\ \hline
         FB-NET & 41 & 75.1 \\ \hline
         \textbf{Ours 30 ms} & \textbf{32} & \textbf{76.5} \\ \hline \hline
         TF-NAS-GPU A & 54 & 76.9 \\ \hline
         EfficientNet B0& 48 & \textbf{77.3} \\ \hline 
         MobileNet v2 (x140) & 50 & 76.5 \\ \hline
         \textbf{Ours 40 ms} & \textbf{41} & 77.1 \\ \hline
    \end{tabular}
    \caption{Imagenet Accuracy vs Latency on NVIDIA P100 GPU for a batch size of 64}
    \label{tab:exp_GPU}
\end{table}



\subsection{Effect of the projection}\label{sec:projection_effect}
As described in section \ref{sec:method}, after our method has converged, the continuous encoding of the accuracy might not belong to the original search space. If most methods simply take the arg-max of every encoding vector, this might lead to a sub optimal solution, either with lower or higher latency that required. In table \ref{tbl:projection}, we show the effect of our projection on the latency of the found network. As we can see, using our projection allows us to reach for a network much closer to the desired latency with less than $1$ ms difference with the required latency. This difference is mostly due to the fact that the search space is discrete and there is not always an architecture for every latency.

\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Expected & argmax & Projection
    \\
    \hline
    35 ms & 36 ms & 35 ms \\
    \hline
    40 ms & 42 ms & 40 ms \\
    \hline
    45 ms & 50 ms & 45 ms \\
    \hline
    50 ms & 54 ms & 49 ms \\
    \hline
    55 ms & 58 ms & 54 ms \\
    \hline
    60 ms & 66 ms & 60 ms \\
    \hline
    \end{tabular}
    \caption{Expected and real latency}
    \label{tbl:projection}
\end{table}

==> intro_v0.1.tex <==
\section{Introduction}
With the rise in popularity of Convolutional Neural Networks (CNN), the need for neural networks with fast inference speed and high accuracy, has been growing continuously. At first, manually designed architectures, such as VGG~\cite{VGG} or ResNet~\cite{ResNet}, targeted powerful GPUs as those were the common computing platform for deep CNNs. Many variants of those architectures were the golden standard until the need for deployment on edge devices or standard CPUs emerged. These are more limited computing platforms, calling for the design of lighter architectures. Furthermore, in practical scenarios there are often hard requirements on the real time latency or power consumption. This has spawned a new line of research aimed at finding architectures with both high performance and bounded resource demand. 

In order to deal with real time latency or power consumption constraints of edge devices or CPUs, Neural Architecture Search (NAS) has been aiming for the automatic design of lighter, and yet, highly accurate neural networks. Starting from unconstrained NAS, \cite{zoph2016neural, liu2018darts, cai2018proxylessnas}, a research branch of NAS has evolved, focusing on meeting a target latency over different platforms, e.g. TPU, CPU, Edge-GPU, FPGA, etc. While some methods heuristically formulate additional objectives to the loss for roughly controlling the latency \cite{tan2019mnasnet,fbnet, effnet, mobilenetv3}, or other indirect proxies such as FLOPS/MACS \cite{SNAS}, more recent methods aim for a strict satisfaction of latency constraints \cite{OFA, TF-NAS}. Latency constrained NAS aims at searching for the most accurate architecture that fully satisfies constraints over its inference time. 
The underlying constraints have to do with (1) the architecture admitting certain structural rules and (2) the resulted latency being lower than some upper bound.

Previous latency constrained NAS methods can be grouped into two categories: Reward based methods such as Reinforcement-Learning (RL) or Evolutionary Algorithm (EA) \cite{OFA,tan2019mnasnet, effnet, mobilenetv3}, where the search is performed by sampling several networks evaluated over some partial validation set to estimate the accuracy and latency forming a reward function. Latency-aware gradient based methods \cite{TF-NAS,fbnet} formulate a differentiable loss function consisting of an accuracy term and a proxy latency penalty term, thus the architecture can be directly optimized using the stochastic gradient descent (SGD) algorithm \cite{SGD} under the resulted trade-off. While the former relay heavily on accuracy and latency predictors that are expensive to acquire and oftentimes inaccurate, the latter incorporate a hard to tune trade-off between accuracy and latency that deteriorates the resulted accuracy without the latency requirement being fully met. This latency constraint is further violated due to the final discretization step projecting the resulted architecture from the differentiable search space to the discrete space of architectures.
 
In this paper, we propose a search algorithm that produces more accurate architectures for a strictly satisfied latency requirement (figure \ref{fig:acc_nas}), while maintaining a scalable search time to many platforms. The proposed algorithm is based on several key ideas, with the goal of formulating the problem more accurately, making less harmful assumptions, and fewer heuristics. 

 This is achieved by constructing a search space capable of parameterizing neural architectures with different operations, widths and depths in a fully differentiable manner. This space induces a one-shot model that is easy to train due to our novel multipath sampling over batch technique, such that every extracted sub-network is properly pretrained. We further suggest an accurate formula for the expected latency of every architecture residing in that space. Thus following a single straight forward pretraining of the one-shot model, we freeze the model's weights and search the space by iteratively solving a constrained optimization problem using the block coordinate stochastic Frank-Wolfe (BC-SFW) algorithm \cite{SFW,BCFW} while tightly satisfying the latency constraint anytime along the search, including the final discretization step, yet converges faster than SGD.
 
 Since the search is over a relatively small number of parameters, governing only the structure of the architecture, the efficient single pretrainig for all target platforms, followed by a fast search for every platform and latency requirement make our solution also scalable for many target devices and latency demands. 
 We believe that our formulation of NAS as a constrained optimization problem, equipped with efficient algorithms to be solved, will give raise to following work incorporating a variety of resource and structural constraints over the search space. 

==> method_v0.tex <==
\section{Method}
\label{sec:method}
In the scope of this paper, we focus on time-constrained NAS, that searches for an architecture with the highest accuracy on a validation set under predefined inference time constraint denoted $T$. The accuracy of a neural network not being differentiable, we replace our objective with a proxy one that is the cross entropy loss over a validation set. Our architecture search space is parametrized by $\balpha$, its associated architecture and weights by $\mathcal{N}(\balpha)$ and $W$, and the objective loss is denoted $\mathcal{L}$. $\mathcal{D}_{T}$ and $\mathcal{D}_{V}$ represent respectively the training and validation sets.
Using these notations, a latency-constrained NAS can be expressed as a bilevel optimization problem and be written as:
\begin{equation}
\label{eqn:NAS_bilevel}
\begin{array}{l}
\displaystyle{\min_\alpha \mathbb{E}_{x \in\mathcal{D}_{V}}\left[\mathcal{L}(W^*, \alpha, x)\right]}\\
\text{s.t.} \\
\displaystyle{W^*=\argmin_{W} \mathbb{E}_{x \in\mathcal{D}_{T}}\left[\mathcal{L}(W, \alpha, x)\right]} \\
\text{inference time}(\mathcal{N}(\alpha))\leq T
\end{array}
\end{equation}
Our method optimizes the above problem using Franck-Wolf algorithm, that performs the optimization in the tangent plane of the constraint hyperplane, expressing every step of the Stochastic Gradient Descent as a bloc coordinate linear programming descent. We start first by describing our search space:
\subsection{Search Space}
Our network architecture search space is composed of a succession of resolution stages, each of them having a maximum possible amount of layers (or block-operations), at a fixed resolution. Each of the layer at every stage consists of a block-operation to be selected among a predefined set of operations (e.g. Bottleneck block, Inverted Residual block, or Identity operation). For every $i^\text{th}$ layer of $s^\text{th}$ stage, a one-hot vector $\balpha_{:i}^s$ encodes the selected block-operation to be chosen while for every $s^\text{th}$ stage, another one-hot vector $\bbeta^s$ encodes the chosen number of layers using the concept of sink point introduced in TF-NAS, as described in Figure \ref{fig:super_net}. 

\begin{figure}[h]
    \centering
  \subfloat[Block Selection \label{fig:block_slect}]{\includegraphics[height=0.11\textheight]{images/operation_selection.pdf}}\quad \subfloat[Elastic network with sink point\label{fig:sink_point}]{\includegraphics[height=0.11\textheight]{images/sink_point.pdf}}
\caption{Super Network}
\label{fig:super_net}
\end{figure}

Our search space is composed of MobileNet Inverted Residual Blocks with the following different possibilities:
    Expansion ratio $er$ in $\{3, 4, 6\}$,
    Kernel Size $k$ in $\{3, 5\}$,
    Squeeze and Excitation ratio $se$ in $\{0, 0.25\}$,
    Depth of every stage $d$ in $\{2,3,4\}$.
The overall size of our search space is:
$((5\times 2\times 2)^2+(5\times 2 \times 2)^3+(5\times 2\times 2)^4)^5\approx 1\times 10^{26}$
In order to avoid the problem of co-adaptation by directly searching for $\balpha, \bbeta$, we parametrize them using a Gumbel-Softmax parametrization. 
In order to avoid redundancy in the different blocks of the architecture, we use the concept of shared weight, and introduce a Slimmable Inverted Residual Block (SIRB), as presented in Fig \ref{fig:inverted_res}. The Point-Wise Expansion and Projection convolutions have shared weights with all possible blocks, and the expansion ratio is selected through a binary mask at the output of the Point-Wise Expansion convolution. To every expansion ratio and kernel is assigned a privatized batch norm as done in [cite Slimmable]. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/elastic_block.pdf}
    \caption{Slimmable Inverted Residual Block (SIRB), blue entries represent the kernels and channels common both for $e_r=1$ and $e_r=1.5$ while red entries represent the ones corresponding to $e_r=1.5$.}
    \label{fig:inverted_res}
\end{figure}

The SIRB reduces the co-adaptation but also boosts the training speed since the number of parameters and amount of stochastic paths of the network is much smaller.

\subsection{Formalization of the problem}
 Denoting by $t^s_{ki}$ the inference time of the $k^\text{th}$ block-operation of the $i^\text{th}$ block from the $s^\text{th}$ stage,  the NAS optimization problem can then be rewritten as:
\begin{equation}
\label{eqn:nas_linear_const}
\begin{array}{l}
\displaystyle{\min_{\balpha, \bbeta}\mathbb{E}_{x \in\mathcal{D}_{V}}\left[\mathcal{L}(W^*, \balpha,\bbeta, x)\right]}\\
\text{s.t.} \\
\displaystyle{W^*=\argmin_{W} \mathbb{E}_{x \in\mathcal{D}_{T}}\left[\mathcal{L}(W, \balpha, \bbeta, x)\right]} \\
\displaystyle{\sum_{s,i,k}t^s_{k,i}\balpha^s_{k,i}\left(\sum_{i\leq j}\bbeta^s_j\right)\leq T} \\
\displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1~~\forall s,i} 
\\
(\balpha^s_{k,i},
\bbeta^s_i)\in\{0,1\}^2~~\forall s,k,i \\
\end{array}
\end{equation}

It is common practice to solve problem (\ref{eqn:nas_linear_const}) by parametrizing the vectors $\bbeta^s_{i}, \balpha^s_{k,i}$ using softmax representation and by adding a soft or hard penalty function to handle the time constraint. This relaxation leads to sub-optimal solution since the $\bbeta^s_{i}$ and  $\balpha^s_{k,i}$ vectors are not necessarily one hot, due to the softmax expression, and projecting them back as performed in [cite TF-NAS] can lead to a solution that does not strictly obey the time constraint. In addition, using a soft penalty requires to select a parameter that accounts for the trade off between the inference time and the final accuracy of the selected network.
Instead, we propose to directly optimize the problem by performing SGD in the constraint hyperplane, using Franck-Wolfe Method. 

\subsection{Franck-Wolfe Algorithm}
Suppose $\mathcal{D}$ is a compact convex set in a vector space and $f \colon \mathcal{D} \to \mathbb{R}$ s a convex, differentiable real-valued function. The Frank-Wolfe algorithm solves the optimization problem:
\begin{equation}
    \label{eqn:FW}
    \min_{\mathbf{x} \in \mathcal{D}}f(\mathbf{x}).
\end{equation}
To do so, at iteration $k+1$, it aims to solve:
\begin{equation}
    \label{eqn:FW2}
    \min_{\mathbf{x_k+\bdelta} \in \mathcal{D}}f(\mathbf{x_k+\bdelta}).
\end{equation}
Using a first order taylor expansion of $f$, we approximate  (\ref{eqn:FW2}) in the neighborhood of $f(x_k)$. The problem could be rewritten as:
\begin{equation}
    \label{eqn:FW3}
    \min_{\mathbf{x_k+\bdelta} \in \mathcal{D}}\bdelta^T\nabla f(\mathbf{x_k})
\end{equation}
Replacing $\bdelta$ with $\gamma (\bs-\mathbf{x_k})$, for $0\leq\gamma\leq 1$ the problem is equivalent to \begin{equation}
    \label{eqn:FW4}
    \min_{\mathbf{\mathbf{x_k}+\gamma (\bs-\mathbf{x_k})} \in \mathcal{D}}(\gamma (s-\mathbf{x_k}))^T\nabla f(\mathbf{x_k}).
\end{equation}
Since $\mathcal{D}$ is convex and we assume that $\mathbf{x_k} \in \mathcal{D}$, the expression $\mathbf{x_k}+\gamma (\bs-\mathbf{x_k}) \in \mathcal{D}$ is equivalent to 
$\bs\in \mathcal{D}$, such as (\ref{eqn:FW3}) can we rewritten as
\begin{equation}
    \label{eqn:FW_step}
    \min_{\mathbf{s} \in \mathcal{D}}s^T\nabla f(\mathbf{x_k}).
\end{equation}
$\mathbf{x}_{k+1}$ is then updated with  
\begin{equation}
\label{eqn:FW_update}
\mathbf{x}_{k+1}\leftarrow \mathbf{x}_k+\gamma(\mathbf{s}_k-\mathbf{x}_k).
\end{equation}
In other words, it iteratively solves the optimization problem in the neighborhood of $\mathbf{x}_k$ by using first-order Taylor approximation of $f$. 
When the function $f$ depends on two variables $\mathbf{x}^{(1)}$ and $\mathbf{x}^{(2)}$, the Block-Coordinate Franck-Wolfe algorithm iteratively solves the optimization problem by first letting $\mathbf{x}^{(1)}$ fixed and optimizing for $\mathbf{x}^{(2)}$ and the opposite for the next step. An example of application of FW algorithm in the context of quadratic programming and its comparison for convergence with regular GD with hard penalty is shown in section \ref{subsec:toy_example}. In addition, in Theorem \ref{theo:softmax_vs_fw}, we show that using Franck-Wolfe algorithm when handling a constrained space instead of a continuous surjective mapping to the constraint space itself leads to better property of convergence and avoid to fine tune the choice of the mapping or its parameters (such as the temperature of the softmax mapping to the simplex).
% \subsection{Multiple Choice Knapsack}
% The Multiple Choice knapsack  problem can be expressed as follows
% $$
% \begin{array}{l}
% \displaystyle{\max\sum_{i=1}^k \sum_{j\in N_i}} p_{ij} \boldsymbol{\alpha}_{ij} \\
% \text{subject to} \\
% \displaystyle{\sum_{i=1}^k\sum_{j\in N_i} t_{ij} \boldsymbol{\alpha}_{ij} \leq T,} \\
% \displaystyle{\sum_{j \in N_i}\boldsymbol{\alpha}_{ij} = 1,\forall~ 1 \leq i \leq k} \\
% \displaystyle{\boldsymbol{\alpha}_{ij} \in \{0,1\}, \forall~ 1 \leq i \leq k, \forall j \in N_i}
% \end{array}
% $$


\subsection{Strong Pretraining}
Problem (\ref{eqn:nas_linear_const}) is a bi-level optimization problem, where both the weights $W^*$ and the architecture parameters $\balpha,\bbeta$ are jointly optimized. It involves two objectives, the outer objective (searching for $\balpha,\bbeta$) and the inner objective (searching for $W$ given $\balpha,\bbeta$). To solve this kind of problem, since it would be computationally prohibitive to compute $W^*$ and its derivative with respect to $\balpha,\bbeta$ for every iteration of the outer optimization problem, several methods exist. For example, [darts] proposes to approximate $\nabla_{\balpha}\mathcal{L}(W^*(\balpha), x)$ with $\nabla_{\balpha}\mathcal{L}(W-\xi\nabla_W\mathcal{L}(W,\balpha), x)$, a common approach in meta learning. Other methods such as [tf-nas] perform alternative steps on $\balpha$ keeping $W$ fixed and then on $W$ keeping $\balpha$ fixed. When updating $W$, the solution might suffer from co-adaptation, meaning that the architecture will be selected according to the weights that have themselves be updated based on current architecture, and it can lead to a very limited exploration of the search space since the architecture and weights would converge to a local minima. Instead, in our method, we first train our SIRB-based elastic network to get a very robust pretrained network with weight $W^*$, such as the accuracy of every extracted sub-network keeping the weights $W^*$ fixed would be close to $\argmin_{W} \mathbb{E}_{x \in\mathcal{D}_{T}}\left[\mathcal{L}(W, \balpha, \bbeta, x)\right]$. In order to to so, we start to train the highest possible network ($d=4, er=6, k=5, se=0.25$), during 250 epochs. Next, we initialize the super-network with the weights from the highest network, and fine-tune the super-network for 100 epochs. During the fine-tuning, unlike most methods that sample a single path in the super-network per GPU-batch of data, we instead sample a different path for every image of the batch, leading to a much higher diversity in the sampling strategy, and allowing us to work with only 8 GPU (unlike OFA that requires 32 GPUS). Then, during the first stage of the architecture search, the weights are not updated. We instead solve the problem:
\begin{equation}
\label{eqn:nas_linear_const_no_W}
\begin{array}{l}
\displaystyle{\min_{\balpha, \bbeta}\mathbb{E}_{x \in\mathcal{D}_{V}}\left[\mathcal{L}(W^*, \balpha,\bbeta, x)\right]}\\
\text{s.t.} \\
\displaystyle{\sum_{s,i,k}t^s_{k,i}\balpha^s_{k,i}\left(\sum_{i\leq j}\bbeta^s_j\right)\leq T} \\
\displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1~~\forall s,i} 
\\
(\balpha^s_{k,i},
\bbeta^s_i)\in\{0,1\}^2~~\forall s,k,i \\
\end{array}
\end{equation}

Once the algorithm as converged, we proceed as other methods, and optimizes both for $W$ and $\balpha,\bbeta$, allowing to change the weights close to our point of convergence. 
\subsection{Method}
Problem (\ref{eqn:nas_linear_const_no_W}) has a quadratic constraint ${\sum_{s,i,k,j\geq i}t^s_{k,i}\balpha^s_{k,i}\bbeta^s_j\leq T}$, that can be reformulated as $\balpha^T\Q\bbeta \leq T$ for some matrix $Q$ with positive coefficients. Applying Franck-Wolfe algorithm to solve (\ref{eqn:nas_linear_const}) leads to the following optimization problem:

\begin{equation}
\label{eqn:nas_linear_const2}
\begin{array}{l}
\displaystyle{\min_{\balpha, \bbeta} \mathbb{E}\left[\balpha^T\nabla_{\balpha}\mathcal{L}+\bbeta^T\nabla_{\bbeta}\mathcal{L}\right]}\\
\text{s.t.} \\
\balpha^T\Q\bbeta \leq T
 \\
\displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1}
\\
(\balpha^s_{k,i},
\bbeta^s_i)\in\{0,1\}^2
\\
\forall s,k,i.
\end{array}
\end{equation}
\paragraph{FW solver} The above problem can be solved using block coordinate descent on $\balpha, \bbeta$, leading to two problems:


\begin{minipage}{0.23\textwidth}
\begin{equation}
\label{eqn:nas_linear_const_alpha}
\begin{array}{l}
\displaystyle{\min_{\balpha} \mathbb{E}\left[\balpha^T\nabla_{\balpha}\mathcal{L}\right]}\\
\text{s.t.} \\
\balpha^T\Q\bbeta \leq T
 \\
\displaystyle{\sum_k \balpha^s_{k,i}=1} 
\\
\balpha^s_{k,i}\in\{0,1\}
\\
\forall s,k,i
\end{array}
\end{equation}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\begin{equation}
\label{eqn:nas_linear_const_beta}
\begin{array}{l}
\displaystyle{\min_{\bbeta} \mathbb{E}\left[\bbeta^T\nabla_{\bbeta}\mathcal{L}\right]}\\
\text{s.t.} \\
\balpha^T\Q\bbeta \leq T
 \\
\displaystyle{\sum_i \bbeta^s_{i}=1}
\\
\bbeta^s_{i}\in\{0,1\}
\\
\forall s,i.
\end{array}
\end{equation}
\end{minipage}

When $\balpha$ or $\bbeta$ are fixed, problem (\ref{eqn:nas_linear_const2}) is nothing but the expression of a Multiple Choice Knapsack Problem (MCKP) and can be solved either with linear programming or with a greedy algorithm. 
As for Block-Coordinate Franck-Wolfe, we alternatively solve for $\balpha$ and $\bbeta$ until convergence. This steps requires very few iterations and every iteration solves a MCKP problem with a linear solver that converges in few milliseconds. 
\paragraph{Initialization} Since FW requires to start from a feasible solution, instead of starting from a random projection in the feasible domain, we seek to start from the most "balanced" initialization, meaning that we want the initial $\balpha, \bbeta$ to be as uniform as possible while respecting the constraints. In order to do so, we solve iteratively the following problems:


\begin{minipage}{0.23\textwidth}
\begin{equation}
\label{eqn:nas_init_alpha}
\begin{array}{l}
\displaystyle{\min_{\balpha}\sum_{s,k,i}(\balpha^s_{k,i}-\balpha^s_{(k-1),i})^2}\\
\text{s.t.} \\
\balpha^T\Q\bbeta \leq T
 \\
\displaystyle{\sum_k \balpha^s_{k,i}=1} 
\\
\balpha^s_{k,i}\in\{0,1\}
\\
\forall s,k,i
\end{array}
\end{equation}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\begin{equation}
\label{eqn:nas_init_beta}
\begin{array}{l}
 \displaystyle{\min_{\bbeta}\sum_{s,i}(\bbeta^s_{i}-\bbeta^s_{i-1})^2}\\
\text{s.t.} \\
\balpha^T\Q\bbeta \leq T
 \\
\displaystyle{\sum_i \bbeta^s_{i}=1}
\\
\bbeta^s_{i}\in\{0,1\}
\\
\forall s,i.
\end{array}
\end{equation}
\end{minipage}



\paragraph{Projection} After the algorithm has converged, the solution might not be binary, due to the update procedure (\ref{eqn:FW_update}). Instead of taking the argmax of every $\balpha,\bbeta$ as done in [TAS] that could lead to an subotpimal solution or violating the time constraint, we solve another linear programming problem with the same constraints as in (\ref{eqn:nas_linear_const_alpha}), (\ref{eqn:nas_linear_const_beta}), and where the objective is replaced with the current $\balpha^k,\bbeta^k$ vectors of the last iteration of the algorithm. 

\begin{minipage}{0.23\textwidth}
\begin{equation}
\label{eqn:nas_linear_const_alpha_final}
\begin{array}{l}
\displaystyle{\min_{\balpha} \mathbb{E}\left[\balpha^T\balpha^k\right]}\\
\text{s.t.} \\
\balpha^T\Q\bbeta \leq T
 \\
\displaystyle{\sum_k \balpha^s_{k,i}=1} 
\\
\balpha^s_{k,i}\in\{0,1\}
\\
\forall s,k,i
\end{array}
\end{equation}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\begin{equation}
\label{eqn:nas_linear_const_beta_final}
\begin{array}{l}
\displaystyle{\min_{\bbeta} \mathbb{E}\left[\bbeta^T\bbeta^{k}\right]}\\
\text{s.t.} \\
\balpha^T\Q\bbeta \leq T
 \\
\displaystyle{\sum_i \bbeta^s_{i}=1}
\\
\bbeta^s_{i}\in\{0,1\}
\\
\forall s,i.
\end{array}
\end{equation}
\end{minipage}



That way, we are searching for an optimal solution that would be as close as possible as the solution after convergence, and that would respect the constraint. Since this problem is a MCKP problem, we have the the guarantee that the obtained solution is binary.


The overall algorithm of the procedure is presented in algorithm \ref{alg:BCFW}.

\begin{algorithm}[tb]
   \caption{Block-Coordinate Franck-Wolf}
   \label{alg:BCFW}
\begin{algorithmic}
\INPUT Validation set $\mathcal{D}_v$, loss function $\mathcal{L}$
\FOR{Data batch $x_V$ {\bfseries in} $\mathcal{D}_V$}
% \FOR{Data batches $(x_T, x_V)$ {\bfseries in} $(\mathcal{D}_T,\mathcal{D}_V)$}

% \STATE Perform SGD step on weights $W$ using $x_T$.

\STATE Compute gradients of $\nabla_{\balpha}\mathcal{L}(x_V), \nabla_{\bbeta}\mathcal{L}(x_V)$ .
\REPEAT 
\STATE Solve alternatively (\ref{eqn:nas_linear_const2}) for $\balpha$ and $\bbeta$ to find solutions $s_{\balpha}, s_{\bbeta}$ using MCKP solver.
\UNTIL{convergence}
\STATE Update $\balpha^{k+1} \leftarrow \balpha^{k}+\gamma(s_{\balpha}-\balpha^{k})$
\STATE Update $\bbeta^{k+1} \leftarrow \bbeta^{k}+\gamma(s_{\bbeta}-\bbeta^{k})$
\ENDFOR
\STATE Solve MCKP problems (\ref{eqn:nas_linear_const_alpha_final}), (\ref{eqn:nas_linear_const_beta_final}) to get optimal solution $\balpha, \bbeta$.
\OUTPUT $\balpha, \bbeta$

%   \STATE {\bfseries Input:} data $x_i$, size $m$
%   \REPEAT
%   \STATE Compute 
%   \FOR{$i=1$ {\bfseries to} $m-1$}
%   \IF{$x_i > x_{i+1}$}
%   \STATE Swap $x_i$ and $x_{i+1}$
%   \STATE $noChange = false$
%   \ENDIF
%   \ENDFOR
%   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}



==> method_v1.tex <==

\section{Method}
\label{sec:method}
In the scope of this paper, we focus on latency-constrained NAS, searching for an architecture with the highest validation accuracy under a predefined latency constraint, denoted by $T$. Our architecture search space $\mathcal{S}$ is parametrized by $\zeta\in\mathcal{S}$, governing the architecture structure in a fully differentiable manner, and $w$, the convolution weights.
A latency-constrained NAS can be expressed as the following constrained bilevel optimization problem:
\begin{align}
&\min_{\zeta \in \mathcal{S}}  \mathbb{E}_{\begin{array}{c}
 x, y \sim\mathcal{D}_{val} \\
\hat{\zeta} \sim \mathcal{P}_\zeta(\mathcal{S})
\end{array}}[\mathcal{L}_{CE}(x, y \mid w^*, \hat{\zeta})] \notag\\
\label{eqn:NAS_bilevel}
&\text{s.t. } 
\text{LAT}(\zeta)\leq T \\
&w^*=\argmin_{w} \mathbb{E}_{\begin{array}{c}
 x, y \sim\mathcal{D}_{train} \\
\hat{\zeta} \sim \mathcal{P}_\zeta(\mathcal{S})
\end{array}}[\mathcal{L}_{CE}(x, y \mid w, \hat{\zeta}) ]\notag
\end{align}
where $\mathcal{D}_{train}$ and $\mathcal{D}_{val}$ are the train and validation sets' distributions respectively, $\mathcal{P}_\zeta(\mathcal{S})$ is some probability measure over the search space parameterized by $\zeta$, $\mathcal{L}_{CE}$ is the cross entropy loss as a differentiable proxy for the negative accuracy and $LAT(\zeta)$ is the estimated latency of the model.

To solve problem~\eqref{eqn:NAS_bilevel}, we construct a fully differentiable search space parameterized by $\zeta=(\balpha, \bbeta)$ (Section~\ref{sec:search_space}), that enables the formulation of a differentiable closed form formula expressing the estimated latency $LAT(\balpha, \bbeta)$ (Section~\ref{sec:latency_formula}) and efficient acquisition of $w^*$ (Section~\ref{sec:inner_problem}). Finally, we introduce rigorous constrained optimization techniques for solving the outer level problem (Section~\ref{sec:outer_problem}).

\subsection{Search Space}
\label{sec:search_space}
Aiming at the most accurate latency, a flexible search space is composed of micro search space that controls the internal structures of each block $b\in\{1,..,d=4\}$, together with the way those are connected to one another in every stage $s\in\{1,..,S=5\}$, forming a macro search space.

\subsubsection{Micro-Search}\label{sec:micro_search}
Every block is an \textit{elastic} version of the MBInvRes block, introduced in~\cite{mobilenetv2}, with expansion ratio $er\in\mathcal{A}_{er}=\{3,4,6\}$ of the point-wise convolution, kernel size $k\in\mathcal{A}_{k}=\{3\times3, 5\times5\}$ of the depth-wise separable convolution (DWS), and Squeeze-and-Excitation (SE) layer~\cite{SE} $se\in\mathcal{A}_{se}=\{\text{on}, \text{off}\}$.
The blocks are configurable, as illustrated at the bottom of Figure~\ref{fig:super_net}, using a parametrization $(\alpha^s_{b,er}, \alpha^s_{b,k}, \alpha^s_{b,se})$, defined for every block $b$ of stage $s$:
\begin{align*}
    \alpha^s_{b,er\setminus k \setminus se}\in \{0, 1\}  \quad \forall er\in\mathcal{A}_{er},\, k \in \mathcal{A}_{k},\, se\in \mathcal{A}_{se}
    \\
    \Sigma_{er \in \mathcal{A}_{er}} \alpha^s_{b,er} = 1
    \, ; \,
    \Sigma_{k \in \mathcal{A}_{k}} \alpha^s_{b,k} = 1
    \,; \,
    \Sigma_{se \in \mathcal{A}_{se}} \alpha^s_{b,k} = 1
\end{align*}
% \begin{align*}
    % \alpha^s_{b,er}\in \{0, 1\}^{\left|\mathcal{A}_{er}\right|} \quad &; \quad \Sigma_{er \in \mathcal{A}_{er}} \alpha^s_{b,er} = 1 \\ 
    % \alpha^s_{b,k}\in \{0, 1\}^{\left|\mathcal{A}_{k}\right|} \quad &; \quad \Sigma_{k \in \mathcal{A}_{k}} \alpha^s_{b,k} = 1 \\
    % \alpha^s_{b,se} \in \{0, 1\}^{\left|\mathcal{A}_{se}\right|} \quad &; \quad
    %  \Sigma_{se\in \mathcal{A}_{se}} \alpha^s_{b,se} = 1
% \end{align*}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{images/search_space.pdf}
\caption{The search space viewed via the one-shot model}
\label{fig:super_net}
\end{figure}
%
%
Each triplet $(er, k, se)$ induces a block configuration $c$ that resides within a micro-search space $\mathcal{C}=\mathcal{A}_{er}\otimes\mathcal{A}_{k}\otimes\mathcal{A}_{se}$, parameterized by  $\balpha\!\in\!\mathcal{A}=\bigotimes_{s=1}^S\bigotimes_{b=1}^d\bigotimes_{c\in\mathcal{C}}\alpha^s_{b,c}$, where $\otimes$ denotes the Cartesian product. Hence, for each block $b$ of stage $s$ we have:
\begin{align*}
    \alpha^s_{b,c}\in \{0, 1\}^{\left|\mathcal{C}\right|} \quad &; \quad 
    \Sigma_{c\in\mathcal{C}} \alpha^s_{b,c} = 1
\end{align*}
An input feature map $x^s_b$ to block $b$ of stage $s$ is processed as follows:
\begin{align*}
    x^s_{b+1}=\sum_{c\in\mathcal{C}}\alpha^s_{b,c}\cdot O^s_{b,c}(x^s_b) 
    % \\
    % O^s_{b,c}(x^s_b)=\sum_{er\in\mathcal{A}_{er}}\alpha^s_{b,er}\cdot Conv^{1\times 1}_{1/er}\left(\alph^s_{b,se=off} + \alph^s_{b,se=on}\cdot SE\left(o^s_{b,c}(x^s_b)\right)\right)
    % \\
    % o^s_{b,c}(x^s_b)=\sum_{k\in\mathcal{A}_{k}}\alpha^s_{b, k}\cdot Conv^{k\times k}\left( \sum_{er\in\mathcal{A}_{er}}\alpha^s_{b,er}\cdot Conv^{1\times 1}_{er}(x^s_b)\right)
\end{align*}
where $O^s_{b,c}(\cdot)$ is the operation performed by the elastic MBInvRes block configured according to $c=(er,k,se)$.

Having several configurations $O^s_{b,c}(\cdot)$ share the same values of $\alpha^s_{b,er}$ or $\alpha^s_{b,k}$ or $\alpha^s_{b,se}$ induces weight sharing between the common operations of the associated architectures. This weight sharing is beneficial for solving the inner problem~\eqref{eqn:NAS_bilevel} effectively, as will be discussed in Section~\ref{sec:inner_problem}.
% At forward pass, a configuration is sampled from the Gumble-Softmax distribution \cite{}, similarily to [SNAS, TF-NAS]

\subsubsection{Macro-Search}\label{sec:macro_search}
Inspired by~\cite{TF-NAS, OFA}, the output of each block of every stage is also directed to the end of the stage as illustrated in the middle of Figure~\ref{fig:super_net}. Thus, the depth of each stage $s$ is controlled by the parameters $\bbeta\in\mathcal{B}=\bigotimes_{s=1}^S\bigotimes_{b=1}^d \beta^s_b$, such that:
\begin{align*}
    \beta^s_b\in \{0, 1\}^d \quad &; \quad 
    \Sigma_{b=1}^d \beta^s_b = 1
\end{align*}
%
We get for the depth: $b^s\!\in\!\left\{b\mid\beta^s_b=1, b\in\{1,..,d\}\right\}$, since $x^{s+1}_1=\sum_{b=1}^{d}\beta^s_b\cdot x^s_{b+1}$.


\subsubsection{The Composed Search Space}\label{sec:composed_search_space}
The overall search space is composed of both the micro and macro search spaces parameterized by $\balpha\in\mathcal{A}$ and $\bbeta\in\mathcal{B}$, respectively, such that:
\begin{align}
   \mathcal{S} = \left\{(\balpha, \bbeta)\left\vert
   \begin{array}{c}
    \balpha\in\mathcal{A}, \bbeta\in\mathcal{B}
    \\
     \alpha^s_{b,c}\in \{0, 1\}^{\left|\mathcal{C}\right|} \,; \, 
    \Sigma_{c\in\mathcal{C}} \alpha^s_{b,c} = 1  \\
   \beta^s_b\in \{0, 1\}^d \,; \,  
    \Sigma_{b=1}^d \beta^s_b = 1 
    \\
    \forall s\in\{1,..,S\}, b\in\{1,..,d\},c\in\mathcal{C}
   \end{array}\right.
   \right\}
   \notag
\end{align}

A continuous probability distribution is induced over the space, except for $\alpha^s_{b,c}\in \mathbb{R}_+^{\left|\mathcal{C}\right|}$ and $\beta^s_b\in \mathbb{R}_+^d$ being continuous rather than discrete Boolean.
% \begin{align}
%   \mathcal{P}_\zeta(\mathcal{S}) = \left\{(\balpha, \bbeta)\left\vert
%   \begin{array}{c}
%     \balpha\in\mathcal{A}, \bbeta\in\mathcal{B}
%     \\
%      \alpha^s_{b,c}\in [0, 1]^{\left|\mathcal{C}\right|} \,; \, 
%     \Sigma_{c\in\mathcal{C}} \alpha^s_{b,c} = 1  \\
%   \beta^s_b\in [0, 1]^d \,; \,  
%     \Sigma_{b=1}^d \beta^s_b = 1 
%     \\
%     \forall s\in\{1,..,S\}, b\in\{1,..,d\},c\in\mathcal{C}
%   \end{array}\right.
%   \right\}
%   \notag
% \end{align}
A sample sub-network is drawn $\hat{\zeta}=(\hat{\balpha}, \hat{\bbeta})\sim \mathcal{P}_\zeta(\mathcal{S})$ using the Gumbel-Softmax Trick~\cite{GumbelSM} such that $\hat{\zeta}\in\mathcal{S}$, as specified in~\eqref{eqn:gumbel_alpha} and~\eqref{eqn:gumbel_beta}.
In summary, one can view the parametrization $(\balpha, \bbeta)$ as a composition of probabilities in $\mathcal{P}_{\zeta}(\mathcal{S})$ or as degenerated one-hot vectors in $\mathcal{S}$.

Effectively we include at least a couple of blocks in each stage by setting $\beta^s_1\equiv 0$, hence, the overall size of the search space is:
\begin{align*}
&|\mathcal{S}|=(\sum_{b=2}^d \left|\mathcal{C}\right|^b)^S =
(\sum_{b=2}^d \left|\mathcal{A}_{er}\right|^b\cdot\left|\mathcal{A}_{k}\right|^b\cdot\left|\mathcal{A}_{se}\right|^b)^S \\
&=((3\times 2\times 2)^2+(3\times 2 \times 2)^3+(3\times 2\times 2)^4)^5\approx 10^{27}
\end{align*}


\subsection{Formulating the Latency Constraint}
\label{sec:latency_formula}
%
The expected latency of a block $b$ can be computed by summing over the latency $t^s_{b,c}$ of every possible configuration $c\in\mathcal{A}$:
$\bar{\ell}^s_{b}=\Sigma_{c\in\mathcal{C}} \alpha^s_{b,c} \cdot t^s_{b,c}$.
Thus the expected latency of a stage of depth $b'$ is 
$\ell^s_{b'}=\sum_{b=1}^{b'}\bar{\ell}^s_{b}$.
% \begin{align}\label{eqn:latency_correction}
% \ell^s_{b'}=\sum_{b=1}^{b'}\bar{\ell}^s_{b}
% \end{align}
Taking the expectation over all possible depths yields  
$\ell^s= \sum_{b'=1}^d \beta^s_{b'}\cdot \ell^s_{b'}$ 
and summing over all the stages results in the following formula for the overall latency:
\begin{align}\label{eqn:latency_formula}
   LAT(\balpha, \bbeta) = 
   \sum_{s=1}^S \sum_{b'=1}^d \sum_{b=1}^{b'}\sum_{c\in\mathcal{C}} \alpha^s_{b,c} \cdot t^s_{b,c} \cdot \beta^s_{b'}
\end{align}
% where the summation originated in (\ref{eqn:latency_correction}) 
The computation of $\ell^s_{b'}$ differentiates our latency formulation~\eqref{eqn:latency_formula} from that of~\cite{TF-NAS}. 
%
A nice property of the latency formula is that it can be expressed as a quadratic constraint by constructing a matrix $\Theta\in\mathbb{R}_+^{S\cdot d\cdot|\mathcal{A}|\times S\cdot d}$ from $t^s_{b,c}$, such that,
\begin{align}\label{eqn:latency_matrix}
   LAT(\zeta)=LAT(\balpha, \bbeta) = \balpha^T \Theta \bbeta \quad ; \quad \zeta\in\mathcal{P}_{\zeta}(\mathcal{S})
\end{align}
The quadratic formulation will become useful when designing the optimization algorithm of~\eqref{eqn:NAS_bilevel}. 

Figure~\ref{fig:latency} provides empirical validation of~\eqref{eqn:latency_formula}, showing that in practice the actual and estimated latency are very close on both GPU and CPU. More details on the experiments are provided in Section~\ref{sec:validate_latency}.
\input{latency_graph}



\textbf{Remark:} By replacing the latency measurements $t^s_{b,c}$ with other resources, e.g., memory, FLOPS, MACS, etc., one can use formula~\eqref{eqn:latency_formula} to add multiple hard constraints to the outer problem of~\eqref{eqn:NAS_bilevel}.



\subsection{Solution to the Inner Problem $w^*$}
\label{sec:inner_problem}
%
Several previous work proposed approximated solutions to the unconstrained problem, typically by alternating or simultaneous updates of $w$ and $\zeta$ \cite{liu2018darts, SNAS, cai2018proxylessnas, fbnet, TF-NAS}:
%
\begin{align*}
&\min_{\zeta \in \mathcal{S}} \mathbb{E}\left[\mathcal{L}_{CE}\left(x, y \mid w^*_\zeta, \zeta\right)\right] \notag\\
&\text{s.t. }
w^*_\zeta=\argmin_{w} \mathbb{E}_{\zeta\sim\mathcal{P}_\zeta(\mathcal{S})}\left[\mathcal{L}_{CE}\left(x, y \mid w, \zeta\right)\right] \notag
\end{align*}
%
This approximation approach has several limitations.
First, obtaining a designated $w^*_\zeta$ with respect to every update of $\zeta$ involves a heavy training of a neural network until convergence.
In addition, the approximation creates a bias towards strengthening networks with few parameters since those learn faster, hence, get sampled even more frequently, further increasing the chance to learn faster in a positive feedback manner. Eventually, often overly simple architectures are generated, e.g., consisting of many skip-connections~\cite{P-DARTS, DARTS+}. Several  remedies have been proposed, e.g., temperature annealing, adding uniform sampling, modified gradients and updating only $w$ for a while before  the joint optimization begins~\cite{noy2020asap, fbnet, TF-NAS, nayman2019xnas}. While those mitigate the bias problem, they do not solve it.

We avoid such approximation whatsoever. Instead we obtain $w^*$ of the inner problem of~\eqref{eqn:NAS_bilevel} only once, with respect to a uniformly distributed architecture, sampling $\bar{\zeta}$ from $\mathcal{P}_{\bar{\zeta}}(\mathcal{S})=U(\mathcal{S})$.

This is done by sampling multiple distinctive paths (sub-networks of the super-graph) for every image in the batch in an efficient way (just a few lines of code provided in the supplementary materials), using the Gumbel-Softmax Trick. 
For every feature map $x$ that goes through block $b$ of stage $s$, distinctive uniform random variables $\mathcal{U}^s_{b,c,x}, \mathcal{U}^s_{b,x}\!\sim\!U(0,1)$ are sampled, governing the path undertaken by this feature map:
\begin{align}
    % x^s_{b+1}&=\sum_{c\in\mathcal{C}}\hat{\alpha}^s_{b,c,x_b}\cdot OP^s_{b,c}(x^s_b)
    % \,; \,
    % x^{s+1}_1=\sum_{b=2}^{d+1}\hat{\beta}^s_b\cdot x^s_b
    % \\
    \label{eqn:gumbel_alpha}
    &\hat{\alpha}^s_{b,c,x} = \frac{e^{\log(\alpha^s_{b,c}) -\log(\log(\mathcal{U}^s_{b,c,x}))}}{\sum_{c\in \mathcal{C}} e^{\log(\alpha^s_{b,c}) -\log(\log(\mathcal{U}^s_{b,c,x}))}}
    \\
    \label{eqn:gumbel_beta}
    &\hat{\beta}^s_{b,x} = \frac{e^{\log(\beta^s_b) -\log(\log(\mathcal{U}^s_{b,x}))}}{\sum_{c\in \mathcal{C}} e^{\log(\alpha^s_{b,c}) -\log(\log(\mathcal{U}^s_{b,x}))}}
\end{align}
% \input{multipath_code}

% \begin{theorm}[Multipath] Given a batch size $n$ and number of machines $m$, the probability of sampling the same path more than once per update step is $1-n\cdot m$
% \end{theorm}
% \begin{proof}
% The number of paths to sample from with replacement at each update step is as big as the size of the search space $|\mathcal{S}|\approx 10^{27}$ (see section \ref{sec:composed_search_space}).
% Following the multipath approach, the number of paths to sample at each update step are the number of input feature maps fed to the model $n\cdot m$.
% Since a path is sampled uniformly with replacement, the number of times a certain path is sampled $Y_p$ admits a Bernoulli distribution $Y_p\sim Bern(n\cdot m, 1/|\mathcal{S}|)$. Hence $\mathbb{P}(Y_p\geq2)$
% \end{proof}

This simple approach implies that the number of paths sampled at each update step is as high as the number of images in the batch. This is two orders of magnitude larger than previous methods that sample a single path per update step. Using multiple paths reduces the variance of the gradients with respect to the paths sampled by an order of magnitude. Furthermore, leveraging the weight sharing implied by the structure of the elastic MBInvRes block (Section~\ref{sec:micro_search}), the number of gradients observed by each operation is increased by a factor of at least $\frac{|\mathcal{C}|}{\max(|\mathcal{A}_{er}|,|\mathcal{A}_{k}|,|\mathcal{A}_{se}|)}=\frac{3\times2\times2}{\max(3,2,2)}\approx 4$. This further reduces the variance by half. 

\input{kendall_tau}
Figure~\ref{fig:acc_kendal_tau} shows that we obtain a one-shot model $w^*$ with high correlation between the ranking of sub-networks directly extracted from it and the corresponding stand-alone counterpart trained from scratch. See more details in Section~\ref{sec:evaluate_inner}. This implies that $w^*$ captures well the quality of sub-structures in the search space.

\subsection{Solving the Outer Problem}
\label{sec:outer_problem}
Having defined the formula for the latency LAT$(\zeta)$ and obtained a solution for $w^*$, we can now continue to solve the outer problem~\eqref{eqn:NAS_bilevel}. 

\subsubsection{Searching the Space}\label{sec:searching_the_space}
As commonly done for gradient based approaches, e.g.,~\cite{liu2018darts}, we relax the discrete search space $\mathcal{S}$ to be continuous by searching for $\zeta\in \mathcal{P}_\zeta(\mathcal{S})$.

Several previous methods proposed solutions to the unconstrained outer problem:
\begin{align}
\min_{\bar{\zeta}} \mathbb{E}_{
 x, y \sim\mathcal{D}_{val} 
% \begin{array}{c}
%  x, y \sim\mathcal{D}_{val} \\
% \hat{\zeta} \sim \mathcal{P}_{g(\bar{\zeta})}(\mathcal{S})
% \end{array}
}\left[\mathcal{L}_{CE}\left(x, y \mid w^*, g(\bar{\zeta})\right)\right]
\end{align}
The common approach is to apply SGD over an unconstrained set of real variables $\bar{\zeta}\!\in\!\mathbb{R}^n$ mapped to the structured search space by $g:\mathbb{R}^n\rightarrow \mathcal{P}_\zeta(\mathcal{S})$.
The update step is set as
$\bar{\zeta}_{t+1} = \bar{\zeta}_t - \gamma_t\nabla_{\bar{\zeta}_t}\mathcal{L}_{CE}\left(x_t, y_t \mid w^*, g(\bar{\zeta}_t)\right)$, 
% \begin{align}\label{eqn:sgd_step}
% \bar{\zeta}_{t+1} = \bar{\zeta}_t - \gamma_t\nabla_{\bar{\zeta}_t}\mathcal{L}_{CE}\left(x_t, y_t \mid w^*, g(\bar{\zeta}_t)\right)
% \end{align}
where $(x_t, y_t)$ and $\gamma_t$ are the sampled data and the learning rate at step $t$, respectively. $g$ is chosen to be either the softmax~\cite{liu2018darts, DARTS+} or the Gumbel-softmax function~\cite{SNAS, fbnet,TF-NAS}. %similarly to (\ref{eqn:gumbel_alpha}), (\ref{eqn:gumbel_beta}).

Instead, we suggest to leverage the convexity of $\mathcal{P}_\zeta(\mathcal{S})$, to directly solve the constrained outer problem:
\begin{align}\label{eqn:constrained_outer_problem}
&\min_{\zeta \in \mathcal{P}_\zeta(\mathcal{S})} \mathbb{E}_{x, y \sim\mathcal{D}_{val}}\left[\mathcal{L}_{CE}\left(x, y \mid w^*, \zeta\right)\right] 
% \\
% &\text{s.t. LAT}(\zeta)\leq T
\end{align}
This can be solved with the stochastic Frank-Wolfe (SFW) algorithm~\cite{SFW} over a set of variables $\bar{\zeta}\in\mathcal{P}_\zeta(\mathcal{S})$, with the following update step:
\begin{align}\label{eqn:sfw_step}
% \zeta_{t+1} &= \zeta_t - \gamma_t(\zeta_t - \xi_t)\\
\zeta_{t+1} &= (1-\gamma_t)\cdot\zeta_t + \gamma_t\cdot\xi_t\\
\xi_t&=\argmin_{\zeta \in \mathcal{P}_\zeta(\mathcal{S})}\zeta^T\cdot \nabla_{\zeta_t}\mathcal{L}_{CE}\left(x_t, y_t \mid w^*, \zeta_t\right)
\label{eqn:lp}
\end{align}
The linear program~\eqref{eqn:lp} can be solved efficiently, e.g., using the Simplex algorithm~\cite{simplex}.

The convexity of $\mathcal{P}_\zeta(\mathcal{S})$ together with $\gamma_t\in[0,1]$ satisfy $\zeta_t\in\mathcal{P}_\zeta(\mathcal{S})$ anytime, as long as $\zeta_0\in\mathcal{P}_\zeta(\mathcal{S})$.
% The later is easily satisfied, see section \ref{sec:init_point}.
 We provide a method for satisfying the latter in the supplementary materials.

% The following theorem states that applying the SFW update (\ref{eqn:sfw_step}) decreases the loss function further than applying the SGD update (\ref{eqn:sgd_step}) at a given step.
% \begin{theo}\label{theo:softmax_vs_fw}
% Given a convex set $\mathcal{S}\subset\mathbb{R}^n$, a surjective mapping $g:\mathbb{R}^n\rightarrow \mathcal{S}$ and a function $f:\mathcal{S}\rightarrow \mathbb{R}$, the following holds for all $t$:
% \begin{align*}
% % f\left(x^{sfw}_t\right) \leq f\left(g\left(x^{sgd}_t\right)\right)
% f(x^{sfw}_t) \leq f(g(x^{sgd}_t))
% \end{align*}
% where,
% \begin{align*}
% x^{sfw}_t &= (1-\gamma_t)\cdot x_t + \gamma_t\cdot\xi_t 
% % x^{sfw}_t &= x_t - \gamma_t(x_t-\xi_t) 
% \quad\,\,;\,\, 
% % \quad;\quad
% \xi_t = \min_{x\in\mathcal{S}} x^T\cdot\nabla_{x_t}f(x_t)
% \\
% x^{sgd}_t &= x_t - \gamma_t\nabla_{x_t}f(g(x_t))
% \end{align*}
% % \begin{equation}
% % \label{eqn:toy_const1}
% %      \min_{s\in\mathcal{S}} f(s)
% % \end{equation}
% % and
% % \begin{equation}
% % \label{eqn:toy_const2}
% %      \min_{x} f(g(x))
% % \end{equation}
% % after a step of FW on (\ref{eqn:toy_const1}), the value of $f$ goes lower that after a step of GD on (\ref{eqn:toy_const2}), when using the same learning rate.
% \end{theo}
% Refer to the supplementary materials for the proof.

% \input{fw_algo}
% where here LAT$(\zeta)$ expresses the expected latency of an architecture sampled from $\mathcal{P}_\zeta(\mathcal{S})$, as discussed in section \ref{sec:latency_formula}.

\subsubsection{Searching Under Latency Constraints}
%Most differentiable resource-aware NAS methods account for the resources through shaping the loss function~\cite{fbnet, TF-NAS}. This soft approach does not meet the constraints tightly. 
Our approach directly solves the constrained outer problem~\ref{eqn:constrained_outer_problem}, hence, it enables the strict satisfaction of resource constraints by further restricting the search space, i.e.,
$\mathcal{S}_{LAT}=\{\zeta \mid \zeta\in \mathcal{P}_\zeta(\mathcal{S}), \text{LAT}(\zeta)\leq T\}$.
Experiments supporting this are described in Section~\ref{subsec:toy_example}.
%
The only requirement on $\mathcal{S}_{LAT}$ is to remain convex. Since $\Theta$ in~\eqref{eqn:latency_matrix} is constructed from measured latency, it is not guaranteed to be positive semi-definite, hence, the induced quadratic constraint could make $\mathcal{S}_{LAT}$ non-convex.

To overcome this, we introduce the Block Coordinate Stochastic Frank-Wolfe (BCSFW) Algorithm~\ref{alg:BCSFW}, that combines Stochastic Frank-Wolfe with Block Coordinate Frank-Wolfe~\cite{BCFW}. This is done by forming separated feasible sets at each step, induced by linear constraints only:
\begin{align}
 \balpha_t \in \mathcal{S}^{\balpha}_t&=\{\balpha\mid \balpha\in \mathcal{A},& \bbeta_t^T \Theta^T \cdot \balpha&\leq T\}
 \\
 \bbeta_t \in \mathcal{S}^{\bbeta}_t&=\{\bbeta\mid \bbeta\in \mathcal{B},& \balpha_t^T \Theta \cdot \bbeta&\leq T\}
\end{align}
 This implies that $\zeta_t=(\balpha_t, \bbeta_t)\in\mathcal{S}_{LAT}$ for all $t$.
Moving inside the feasible domain at anytime avoids irrelevant infeasible structures from being promoted and hiding feasible structures.
\input{fw_algo}

%  The following main theorem shows that after $\mathcal{O}(1/\epsilon)$ many steps, Algorithm~\ref{alg:BCSFW} obtains an $\epsilon$-approximate solution to the outer problem (\ref{eqn:NAS_bilevel}), and guaranteed $\epsilon$-small duality gap, in expectation under several assumptions on the loss function.
%  \begin{theo}\label{theo:bcsfw}
%  TODO
%  \end{theo}
% Refer to the supplementary materials for the proof.

% \subsubsection{obtaining a feasible initial point}\label{sec:init_point}
% algorithm \ref{alg:bcsfw} requires a feasible initial point $(\balpha_0, \bbeta_0) \in \mathcal{s}_{lat}$. assuming such a point exists, i.e. as $t$ is large enough, a trivial initial point $(\balpha_0, \bbeta_0):=(\tilde{\balpha}, \tilde{\bbeta})$ is associated with the lightest structure in the search space $\mathcal{s}\subset\mathcal{p}_\zeta(\mathcal{s})$, i.e. setting: 
% \begin{align}\label{eqn:trivial_init}
%     \tilde{\alpha}^s_{b,c}=\mathbbm{1}\{c=1\} \, ; \, \tilde{\beta}^s_b=\mathbbm{1}\{b=2\}
% \end{align} for all $s\in\{1,..,s\}, b\in\{1,..,d\},c\in\mathcal{c}$, where $\mathbbm{1}\{\cdot\}$ is the indicator function.
% however, starting from this point condemns the gradients with respect to all other structures to be always zero due to the way paths are sampled from the space using the gumbel-softmax trick, section \ref{sec:composed_search_space}.

% hence for a balanced propagation of gradients, the closest to uniformly distributed structure in $\mathcal{s}_{lat}$ is encouraged. for this purpose we solve the following quadratic programs (qp) alternately,
% \begin{align}\label{eqn:qp_init}
%   &\min_{\balpha\in\mathcal{s}^{\tilde{\balpha}}} \sum_{s=1}^s \sum_{b=1}^{d-1}\sum_{c=1}^{|\mathcal{c}|-1} (\alpha^s_{b,c+1}-\alpha^s_{b,c})^2 
%   \\
%   &\min_{\bbeta\in\mathcal{s}^{\tilde{\bbeta}}} \sum_{s=1}^s \sum_{b=1}^{d-1}(\beta^s_{b+1}-\beta^s_{b})^2
%   \notag
% %   \min_{(\balpha, \bbeta) \in \mathcal{s}_{lat}} \sum_{s=1}^s \sum_{b=1}^{d-1}\left((\beta^s_{b+1}-\beta^s_{b})^2 + \sum_{c=1}^{|\mathcal{c}|-1} (\alpha^s_{b,c+1}-\alpha^s_{b,c})^2\right)
% \end{align}
% using a qp solver at each step. 

% sorting the indices of configurations according to their measured latency, the objectives in (\ref{eqn:qp_init}) promote probabilities of consecutive indices to be close to each other, forming chains of uniformly distributed probabilities up to an infeasible configuration, there a chain of zero probability if formed.
% %The benefits from starting with such initial point is shown in section \ref{}.

\subsubsection{Projection Back to the Discrete Space}\label{sec:projection}
As differentiable NAS methods are inherently associated with a continuous search space, a final discretizaiton step $\mathbb{P}:\mathcal{P}_\zeta(\mathcal{S})\rightarrow\mathcal{S}$ is required for extracting a single architecture. 
Most methods use the \textit{argmax} operator:
\begin{align}\label{eqn:argmax}
\bar{\alpha}^s_{b,c}&:=\mathbbm{1}\{c=\argmax_{c\in\mathcal{C}}\alpha^s_{b,c}\} 
% \,; \,
\\\notag
\bar{\beta}^s_b&:=\mathbbm{1}\{b=\argmax_{b=2,..,d}\beta^s_b\} 
\end{align}
for all $s\in\{1,..,S\}, b\in\{1,..,d\},c\in\mathcal{C}$, where $(\bar{\balpha}, \bar{\bbeta})$ is the solution to the outer problem of~\eqref{eqn:NAS_bilevel}.
This has been shown in~\ref{eqn:NAS_bilevel} to lead to a significant drop in accuracy, because the weights $w^*$ were tuned during the search, via alternating steps between the inner and outer problem, to fit the last solution which is suddenly changed. 
Several methods mitigate this gap by promoting sparse probabilities during the search, e.g.,~\cite{noy2020asap, nayman2019xnas}.
Our approach completely eliminates the gap, since it can extract a partially trained sub-network from the one-shot model without any degradation, as described in Section~\ref{sec:inner_problem}.

For resource-aware NAS methods, applying such projection results in yet another possible violation of the constraints in place, since it might increase the resources associated with the resulted architecture as demonstrated in section \ref{sec:projection_effect}.

Viewing the solution of the outer problem $(\balpha^*, \bbeta^*)$ as the credit assigned to each configuration,
we introduce a projection step that maximizes the overall credit while strictly satisfying the latency constraints. It is based on solving the following two linear programs:
\begin{align}\label{eqn:projection_step}
  \max_{\balpha\in\mathcal{S}^{\balpha^*}} \balpha^T\cdot \balpha^*
  \quad; \quad
  \max_{\bbeta\in\mathcal{S}^{\bbeta^*}} \bbeta^T\cdot\bbeta^*
\end{align}
Note, that when is no latency constraint, e.g., $T\rightarrow\infty$, \eqref{eqn:projection_step} coincides with~\eqref{eqn:argmax}.

We next provide a theorem that guarantees that the projection~\eqref{eqn:projection_step} yields a sparse solution, representing a valid sub-network of the one-shot model. We rely on the observation that a single probability vector from those composing $\balpha$ and $\bbeta$ contains up to two non-zero entries each, as all the rest are one-hot vectors. 
\begin{theo}
The solution $(\balpha, \bbeta)$ of \eqref{eqn:projection_step} admits:
\begin{align*}
  &\sum_{c\in\mathcal{C}}|\alpha^s_{b,c}|^0 = 1 \,\forall 
  (s, b)\in\{1,..,S\}\otimes \{1,..,d\}\setminus{\{(s_{\balpha}, b_{\balpha})\}}
  \\
  &\sum_{b=1}^d|\beta^s_b|^0 = 1 \quad \forall s\in\{1,..,S\}\setminus{\{s_{\bbeta}\}}
\end{align*}
where $|\cdot|^0=\mathbbm{1}\{\cdot>0\}$ and $(s_{\balpha}$, $b_{\balpha})$, $s_{\bbeta}$  are single block and stage respectively, satisfying:
\begin{align}\label{eqn:dense_remiders}
  \sum_{c\in\mathcal{C}}|\alpha^{s_{\balpha}}_{{b_{\balpha}},c}|^0 \leq 2
  \quad ; \quad 
  \sum_{b=1}^d|\beta^{s_{\bbeta}}_b|^0 \leq 2
\end{align}
\end{theo}
Refer to the supplementary materials for the proof.

\textbf{Remark:} A negligible deviation is associated with taking the argmax~\eqref{eqn:argmax} over the only two couples referred to in~\eqref{eqn:dense_remiders}, see section \ref{sec:projection_effect}. This can be entirely eliminated by solving an equivalent Multiple-Choice Knapsack Problem (MCKP) as described in the supplementary material.


% % \subsection{Formalization of the problem}
%  Denoting by $t^s_{ki}$ the inference time of the $k^\text{th}$ block-operation of the $i^\text{th}$ block from the $s^\text{th}$ stage, once the inner problem has been solved, the NAS optimization problem can then be rewritten as:
% % \begin{equation}
% % \label{eqn:nas_linear_const}
% % \begin{array}{l}
% % \displaystyle{\min_{\balpha, \bbeta}\mathbb{E}_{x \in\mathcal{D}_{V}}\left[\mathcal{L}(W^*, \balpha,\bbeta, x)\right]}\\
% % \text{s.t.} \\
% % \displaystyle{W^*=\argmin_{W} \mathbb{E}_{x \in\mathcal{D}_{T}}\left[\mathcal{L}(W, \balpha, \bbeta, x)\right]} \\
% % \displaystyle{\sum_{s,i,k}t^s_{k,i}\balpha^s_{k,i}\left(\sum_{i\leq j}\bbeta^s_j\right)\leq T} \\
% % \displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1~~\forall s,i} 
% % \\
% % (\balpha^s_{k,i},
% % \bbeta^s_i)\in\{0,1\}^2~~\forall s,k,i \\
% % \end{array}
% % \end{equation}

% \begin{equation}
% \label{eqn:nas_linear_const_no_W}
% \begin{array}{l}
% \displaystyle{\min_{\balpha, \bbeta}\mathbb{E}_{x \in\mathcal{D}_{V}}\left[\mathcal{L}(W^*, \balpha,\bbeta, x)\right]}\\
% \text{s.t.} \\
% \displaystyle{\sum_{s,i,k}t^s_{k,i}\balpha^s_{k,i}\left(\sum_{i\leq j}\bbeta^s_j\right)\leq T} \\
% \displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1~~\forall s,i} 
% \\
% (\balpha^s_{k,i},
% \bbeta^s_i)\in\{0,1\}^2~~\forall s,k,i \\
% \end{array}
% \end{equation}


% It is common practice to solve problem (\ref{eqn:nas_linear_const_no_W}) by parametrizing the vectors $\bbeta^s_{i}, \balpha^s_{k,i}$ using softmax representation and by adding a soft or hard penalty function to handle the time constraint. This relaxation leads to sub-optimal solution since the $\bbeta^s_{i}$ and  $\balpha^s_{k,i}$ vectors are not necessarily one hot, due to the softmax expression, and projecting them back as performed in \cite{TF-NAS} can lead to a solution that does not strictly obey the time constraint. In addition, using a soft penalty requires to select a parameter that accounts for the trade off between the inference time and the final accuracy of the selected network.
% Instead, we propose to directly optimize the problem by performing SGD in the constraint hyperplane, using Franck-Wolfe Method. 

% \subsection{Franck-Wolfe Algorithm}
% Suppose $\mathcal{D}$ is a compact convex set in a vector space and $f \colon \mathcal{D} \to \mathbb{R}$ s a convex, differentiable real-valued function. The Frank-Wolfe algorithm solves the optimization problem:
% \begin{equation}
%     \label{eqn:FW}
%     \min_{\mathbf{x} \in \mathcal{D}}f(\mathbf{x}).
% \end{equation}
% To do so, at iteration $k+1$, it aims to solve:
% \begin{equation}
%     \label{eqn:FW2}
%     \min_{\mathbf{x_k+\bdelta} \in \mathcal{D}}f(\mathbf{x_k+\bdelta}).
% \end{equation}
% Using a first order taylor expansion of $f$, we approximate  (\ref{eqn:FW2}) in the neighborhood of $f(x_k)$. The problem could be rewritten as:
% \begin{equation}
%     \label{eqn:FW3}
%     \min_{\mathbf{x_k+\bdelta} \in \mathcal{D}}\bdelta^T\nabla f(\mathbf{x_k})
% \end{equation}
% Replacing $\bdelta$ with $\gamma (\bs-\mathbf{x_k})$, for $0\leq\gamma\leq 1$ the problem is equivalent to \begin{equation}
%     \label{eqn:FW4}
%     \min_{\mathbf{\mathbf{x_k}+\gamma (\bs-\mathbf{x_k})} \in \mathcal{D}}(\gamma (s-\mathbf{x_k}))^T\nabla f(\mathbf{x_k}).
% \end{equation}
% Since $\mathcal{D}$ is convex and we assume that $\mathbf{x_k} \in \mathcal{D}$, the expression $\mathbf{x_k}+\gamma (\bs-\mathbf{x_k}) \in \mathcal{D}$ is equivalent to 
% $\bs\in \mathcal{D}$, such as (\ref{eqn:FW3}) can we rewritten as
% \begin{equation}
%     \label{eqn:FW_step}
%     \min_{\mathbf{s} \in \mathcal{D}}s^T\nabla f(\mathbf{x_k}).
% \end{equation}
% $\mathbf{x}_{k+1}$ is then updated with  
% \begin{equation}
% \label{eqn:FW_update}
% \mathbf{x}_{k+1}\leftarrow \mathbf{x}_k+\gamma(\mathbf{s}_k-\mathbf{x}_k).
% \end{equation}
% In other words, it iteratively solves the optimization problem in the neighborhood of $\mathbf{x}_k$ by using first-order Taylor approximation of $f$. 
% When the function $f$ depends on two variables $\mathbf{x}^{(1)}$ and $\mathbf{x}^{(2)}$, the Block-Coordinate Franck-Wolfe algorithm iteratively solves the optimization problem by first letting $\mathbf{x}^{(1)}$ fixed and optimizing for $\mathbf{x}^{(2)}$ and the opposite for the next step. An example of application of FW algorithm in the context of quadratic programming and its comparison for convergence with regular GD with hard penalty is shown in section \ref{subsec:toy_example}. In addition, in Theorem \ref{theo:softmax_vs_fw}, we show that using Franck-Wolfe algorithm when handling a constrained space instead of a continuous surjective mapping to the constraint space itself leads to better property of convergence and avoid to fine tune the choice of the mapping or its parameters (such as the temperature of the softmax mapping to the simplex).
% % \subsection{Multiple Choice Knapsack}
% % The Multiple Choice knapsack  problem can be expressed as follows
% % $$
% % \begin{array}{l}
% % \displaystyle{\max\sum_{i=1}^k \sum_{j\in N_i}} p_{ij} \boldsymbol{\alpha}_{ij} \\
% % \text{subject to} \\
% % \displaystyle{\sum_{i=1}^k\sum_{j\in N_i} t_{ij} \boldsymbol{\alpha}_{ij} \leq T,} \\
% % \displaystyle{\sum_{j \in N_i}\boldsymbol{\alpha}_{ij} = 1,\forall~ 1 \leq i \leq k} \\
% % \displaystyle{\boldsymbol{\alpha}_{ij} \in \{0,1\}, \forall~ 1 \leq i \leq k, \forall j \in N_i}
% % \end{array}
% % $$


% % \subsection{Strong Pretraining}
% % Problem (\ref{eqn:nas_linear_const}) is a bi-level optimization problem, where both the weights $W^*$ and the architecture parameters $\balpha,\bbeta$ are jointly optimized. It involves two objectives, the outer objective (searching for $\balpha,\bbeta$) and the inner objective (searching for $W$ given $\balpha,\bbeta$). To solve this kind of problem, since it would be computationally prohibitive to compute $W^*$ and its derivative with respect to $\balpha,\bbeta$ for every iteration of the outer optimization problem, several methods exist. For example, [darts] proposes to approximate $\nabla_{\balpha}\mathcal{L}(W^*(\balpha), x)$ with $\nabla_{\balpha}\mathcal{L}(W-\xi\nabla_W\mathcal{L}(W,\balpha), x)$, a common approach in meta learning. Other methods such as [tf-nas] perform alternative steps on $\balpha$ keeping $W$ fixed and then on $W$ keeping $\balpha$ fixed. When updating $W$, the solution might suffer from co-adaptation, meaning that the architecture will be selected according to the weights that have themselves be updated based on current architecture, and it can lead to a very limited exploration of the search space since the architecture and weights would converge to a local minima. Instead, in our method, we first train our SIRB-based elastic network to get a very robust pretrained network with weight $W^*$, such as the accuracy of every extracted sub-network keeping the weights $W^*$ fixed would be close to $\argmin_{W} \mathbb{E}_{x \in\mathcal{D}_{T}}\left[\mathcal{L}(W, \balpha, \bbeta, x)\right]$. In order to to so, we start to train the highest possible network ($d=4, er=6, k=5, se=0.25$), during 250 epochs. Next, we initialize the super-network with the weights from the highest network, and fine-tune the super-network for 100 epochs. During the fine-tuning, unlike most methods that sample a single path in the super-network per GPU-batch of data, we instead sample a different path for every image of the batch, leading to a much higher diversity in the sampling strategy, and allowing us to work with only 8 GPU (unlike OFA that requires 32 GPUS). Then, during the first stage of the architecture search, the weights are not updated. We instead solve the problem:
% % \begin{equation}
% % \label{eqn:nas_linear_const_no_W}
% % \begin{array}{l}
% % \displaystyle{\min_{\balpha, \bbeta}\mathbb{E}_{x \in\mathcal{D}_{V}}\left[\mathcal{L}(W^*, \balpha,\bbeta, x)\right]}\\
% % \text{s.t.} \\
% % \displaystyle{\sum_{s,i,k}t^s_{k,i}\balpha^s_{k,i}\left(\sum_{i\leq j}\bbeta^s_j\right)\leq T} \\
% % \displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1~~\forall s,i} 
% % \\
% % (\balpha^s_{k,i},
% % \bbeta^s_i)\in\{0,1\}^2~~\forall s,k,i \\
% % \end{array}
% % \end{equation}

% % Once the algorithm as converged, we proceed as other methods, and optimizes both for $W$ and $\balpha,\bbeta$, allowing to change the weights close to our point of convergence. 
% \subsection{Method}
% Problem (\ref{eqn:nas_linear_const_no_W}) has a quadratic constraint ${\sum_{s,i,k,j\geq i}t^s_{k,i}\balpha^s_{k,i}\bbeta^s_j\leq T}$, that can be reformulated as $\balpha^T\Theta\bbeta \leq T$ for some matrix $\Theta$ with positive coefficients. Applying Franck-Wolfe algorithm to solve (\ref{eqn:nas_linear_const_no_W}) leads to the following optimization problem:

% \begin{equation}
% \label{eqn:nas_linear_const2}
% \begin{array}{l}
% \displaystyle{\min_{\balpha, \bbeta} \mathbb{E}\left[\balpha^T\nabla_{\balpha}\mathcal{L}+\bbeta^T\nabla_{\bbeta}\mathcal{L}\right]}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1}
% \\
% (\balpha^s_{k,i},
% \bbeta^s_i)\in\{0,1\}^2
% \\
% \forall s,k,i.
% \end{array}
% \end{equation}
% \paragraph{FW solver} The above problem can be solved using block coordinate descent on $\balpha, \bbeta$, leading to two problems:


% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_linear_const_alpha}
% \begin{array}{l}
% \displaystyle{\min_{\balpha} \mathbb{E}\left[\balpha^T\nabla_{\balpha}\mathcal{L}\right]}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_k \balpha^s_{k,i}=1} 
% \\
% \balpha^s_{k,i}\in\{0,1\}
% \\
% \forall s,k,i
% \end{array}
% \end{equation}
% \end{minipage}
% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_linear_const_beta}
% \begin{array}{l}
% \displaystyle{\min_{\bbeta} \mathbb{E}\left[\bbeta^T\nabla_{\bbeta}\mathcal{L}\right]}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_i \bbeta^s_{i}=1}
% \\
% \bbeta^s_{i}\in\{0,1\}
% \\
% \forall s,i.
% \end{array}
% \end{equation}
% \end{minipage}

% When $\balpha$ or $\bbeta$ are fixed, problem (\ref{eqn:nas_linear_const2}) is nothing but the expression of a Multiple Choice Knapsack Problem (MCKP) and can be solved either with linear programming or with a greedy algorithm. 
% As for Block-Coordinate Franck-Wolfe, we alternatively solve for $\balpha$ and $\bbeta$ until convergence. This steps requires very few iterations and every iteration solves a MCKP problem with a linear solver that converges in few milliseconds. 
% \paragraph{Initialization} Since FW requires to start from a feasible solution, instead of starting from a random projection in the feasible domain, we seek to start from the most "balanced" initialization, meaning that we want the initial $\balpha, \bbeta$ to be as uniform as possible while respecting the constraints. In order to do so, we solve iteratively the following problems:


% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_init_alpha}
% \begin{array}{l}
% \displaystyle{\min_{\balpha}\sum_{s,k,i}(\balpha^s_{k,i}-\balpha^s_{(k-1),i})^2}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_k \balpha^s_{k,i}=1} 
% \\
% \balpha^s_{k,i}\in\{0,1\}
% \\
% \forall s,k,i
% \end{array}
% \end{equation}
% \end{minipage}
% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_init_beta}
% \begin{array}{l}
%  \displaystyle{\min_{\bbeta}\sum_{s,i}(\bbeta^s_{i}-\bbeta^s_{i-1})^2}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_i \bbeta^s_{i}=1}
% \\
% \bbeta^s_{i}\in\{0,1\}
% \\
% \forall s,i.
% \end{array}
% \end{equation}

% \input{fw_algo}
% where here LAT$(\zeta)$ expresses the expected latency of an architecture sampled from $\mathcal{P}_\zeta(\mathcal{S})$, as discussed in section \ref{sec:latency_formula}.




% % \subsection{Formalization of the problem}
%  Denoting by $t^s_{ki}$ the inference time of the $k^\text{th}$ block-operation of the $i^\text{th}$ block from the $s^\text{th}$ stage, once the inner problem has been solved, the NAS optimization problem can then be rewritten as:
% % \begin{equation}
% % \label{eqn:nas_linear_const}
% % \begin{array}{l}
% % \displaystyle{\min_{\balpha, \bbeta}\mathbb{E}_{x \in\mathcal{D}_{V}}\left[\mathcal{L}(W^*, \balpha,\bbeta, x)\right]}\\
% % \text{s.t.} \\
% % \displaystyle{W^*=\argmin_{W} \mathbb{E}_{x \in\mathcal{D}_{T}}\left[\mathcal{L}(W, \balpha, \bbeta, x)\right]} \\
% % \displaystyle{\sum_{s,i,k}t^s_{k,i}\balpha^s_{k,i}\left(\sum_{i\leq j}\bbeta^s_j\right)\leq T} \\
% % \displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1~~\forall s,i} 
% % \\
% % (\balpha^s_{k,i},
% % \bbeta^s_i)\in\{0,1\}^2~~\forall s,k,i \\
% % \end{array}
% % \end{equation}

% \begin{equation}
% \label{eqn:nas_linear_const_no_W}
% \begin{array}{l}
% \displaystyle{\min_{\balpha, \bbeta}\mathbb{E}_{x \in\mathcal{D}_{V}}\left[\mathcal{L}(W^*, \balpha,\bbeta, x)\right]}\\
% \text{s.t.} \\
% \displaystyle{\sum_{s,i,k}t^s_{k,i}\balpha^s_{k,i}\left(\sum_{i\leq j}\bbeta^s_j\right)\leq T} \\
% \displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1~~\forall s,i} 
% \\
% (\balpha^s_{k,i},
% \bbeta^s_i)\in\{0,1\}^2~~\forall s,k,i \\
% \end{array}
% \end{equation}


% It is common practice to solve problem (\ref{eqn:nas_linear_const_no_W}) by parametrizing the vectors $\bbeta^s_{i}, \balpha^s_{k,i}$ using softmax representation and by adding a soft or hard penalty function to handle the time constraint. This relaxation leads to sub-optimal solution since the $\bbeta^s_{i}$ and  $\balpha^s_{k,i}$ vectors are not necessarily one hot, due to the softmax expression, and projecting them back as performed in \cite{TF-NAS} can lead to a solution that does not strictly obey the time constraint. In addition, using a soft penalty requires to select a parameter that accounts for the trade off between the inference time and the final accuracy of the selected network.
% Instead, we propose to directly optimize the problem by performing SGD in the constraint hyperplane, using Franck-Wolfe Method. 

% \subsection{Franck-Wolfe Algorithm}
% Suppose $\mathcal{D}$ is a compact convex set in a vector space and $f \colon \mathcal{D} \to \mathbb{R}$ s a convex, differentiable real-valued function. The Frank-Wolfe algorithm solves the optimization problem:
% \begin{equation}
%     \label{eqn:FW}
%     \min_{\mathbf{x} \in \mathcal{D}}f(\mathbf{x}).
% \end{equation}
% To do so, at iteration $k+1$, it aims to solve:
% \begin{equation}
%     \label{eqn:FW2}
%     \min_{\mathbf{x_k+\bdelta} \in \mathcal{D}}f(\mathbf{x_k+\bdelta}).
% \end{equation}
% Using a first order taylor expansion of $f$, we approximate  (\ref{eqn:FW2}) in the neighborhood of $f(x_k)$. The problem could be rewritten as:
% \begin{equation}
%     \label{eqn:FW3}
%     \min_{\mathbf{x_k+\bdelta} \in \mathcal{D}}\bdelta^T\nabla f(\mathbf{x_k})
% \end{equation}
% Replacing $\bdelta$ with $\gamma (\bs-\mathbf{x_k})$, for $0\leq\gamma\leq 1$ the problem is equivalent to \begin{equation}
%     \label{eqn:FW4}
%     \min_{\mathbf{\mathbf{x_k}+\gamma (\bs-\mathbf{x_k})} \in \mathcal{D}}(\gamma (s-\mathbf{x_k}))^T\nabla f(\mathbf{x_k}).
% \end{equation}
% Since $\mathcal{D}$ is convex and we assume that $\mathbf{x_k} \in \mathcal{D}$, the expression $\mathbf{x_k}+\gamma (\bs-\mathbf{x_k}) \in \mathcal{D}$ is equivalent to 
% $\bs\in \mathcal{D}$, such as (\ref{eqn:FW3}) can we rewritten as
% \begin{equation}
%     \label{eqn:FW_step}
%     \min_{\mathbf{s} \in \mathcal{D}}s^T\nabla f(\mathbf{x_k}).
% \end{equation}
% $\mathbf{x}_{k+1}$ is then updated with  
% \begin{equation}
% \label{eqn:FW_update}
% \mathbf{x}_{k+1}\leftarrow \mathbf{x}_k+\gamma(\mathbf{s}_k-\mathbf{x}_k).
% \end{equation}
% In other words, it iteratively solves the optimization problem in the neighborhood of $\mathbf{x}_k$ by using first-order Taylor approximation of $f$. 
% When the function $f$ depends on two variables $\mathbf{x}^{(1)}$ and $\mathbf{x}^{(2)}$, the Block-Coordinate Franck-Wolfe algorithm iteratively solves the optimization problem by first letting $\mathbf{x}^{(1)}$ fixed and optimizing for $\mathbf{x}^{(2)}$ and the opposite for the next step. An example of application of FW algorithm in the context of quadratic programming and its comparison for convergence with regular GD with hard penalty is shown in section \ref{subsec:toy_example}. In addition, in Theorem \ref{theo:softmax_vs_fw}, we show that using Franck-Wolfe algorithm when handling a constrained space instead of a continuous surjective mapping to the constraint space itself leads to better property of convergence and avoid to fine tune the choice of the mapping or its parameters (such as the temperature of the softmax mapping to the simplex).
% % \subsection{Multiple Choice Knapsack}
% % The Multiple Choice knapsack  problem can be expressed as follows
% % $$
% % \begin{array}{l}
% % \displaystyle{\max\sum_{i=1}^k \sum_{j\in N_i}} p_{ij} \boldsymbol{\alpha}_{ij} \\
% % \text{subject to} \\
% % \displaystyle{\sum_{i=1}^k\sum_{j\in N_i} t_{ij} \boldsymbol{\alpha}_{ij} \leq T,} \\
% % \displaystyle{\sum_{j \in N_i}\boldsymbol{\alpha}_{ij} = 1,\forall~ 1 \leq i \leq k} \\
% % \displaystyle{\boldsymbol{\alpha}_{ij} \in \{0,1\}, \forall~ 1 \leq i \leq k, \forall j \in N_i}
% % \end{array}
% % $$


% % \subsection{Strong Pretraining}
% % Problem (\ref{eqn:nas_linear_const}) is a bi-level optimization problem, where both the weights $W^*$ and the architecture parameters $\balpha,\bbeta$ are jointly optimized. It involves two objectives, the outer objective (searching for $\balpha,\bbeta$) and the inner objective (searching for $W$ given $\balpha,\bbeta$). To solve this kind of problem, since it would be computationally prohibitive to compute $W^*$ and its derivative with respect to $\balpha,\bbeta$ for every iteration of the outer optimization problem, several methods exist. For example, [darts] proposes to approximate $\nabla_{\balpha}\mathcal{L}(W^*(\balpha), x)$ with $\nabla_{\balpha}\mathcal{L}(W-\xi\nabla_W\mathcal{L}(W,\balpha), x)$, a common approach in meta learning. Other methods such as [tf-nas] perform alternative steps on $\balpha$ keeping $W$ fixed and then on $W$ keeping $\balpha$ fixed. When updating $W$, the solution might suffer from co-adaptation, meaning that the architecture will be selected according to the weights that have themselves be updated based on current architecture, and it can lead to a very limited exploration of the search space since the architecture and weights would converge to a local minima. Instead, in our method, we first train our SIRB-based elastic network to get a very robust pretrained network with weight $W^*$, such as the accuracy of every extracted sub-network keeping the weights $W^*$ fixed would be close to $\argmin_{W} \mathbb{E}_{x \in\mathcal{D}_{T}}\left[\mathcal{L}(W, \balpha, \bbeta, x)\right]$. In order to to so, we start to train the highest possible network ($d=4, er=6, k=5, se=0.25$), during 250 epochs. Next, we initialize the super-network with the weights from the highest network, and fine-tune the super-network for 100 epochs. During the fine-tuning, unlike most methods that sample a single path in the super-network per GPU-batch of data, we instead sample a different path for every image of the batch, leading to a much higher diversity in the sampling strategy, and allowing us to work with only 8 GPU (unlike OFA that requires 32 GPUS). Then, during the first stage of the architecture search, the weights are not updated. We instead solve the problem:
% % \begin{equation}
% % \label{eqn:nas_linear_const_no_W}
% % \begin{array}{l}
% % \displaystyle{\min_{\balpha, \bbeta}\mathbb{E}_{x \in\mathcal{D}_{V}}\left[\mathcal{L}(W^*, \balpha,\bbeta, x)\right]}\\
% % \text{s.t.} \\
% % \displaystyle{\sum_{s,i,k}t^s_{k,i}\balpha^s_{k,i}\left(\sum_{i\leq j}\bbeta^s_j\right)\leq T} \\
% % \displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1~~\forall s,i} 
% % \\
% % (\balpha^s_{k,i},
% % \bbeta^s_i)\in\{0,1\}^2~~\forall s,k,i \\
% % \end{array}
% % \end{equation}

% % Once the algorithm as converged, we proceed as other methods, and optimizes both for $W$ and $\balpha,\bbeta$, allowing to change the weights close to our point of convergence. 
% \subsection{Method}
% Problem (\ref{eqn:nas_linear_const_no_W}) has a quadratic constraint ${\sum_{s,i,k,j\geq i}t^s_{k,i}\balpha^s_{k,i}\bbeta^s_j\leq T}$, that can be reformulated as $\balpha^T\Theta\bbeta \leq T$ for some matrix $\Theta$ with positive coefficients. Applying Franck-Wolfe algorithm to solve (\ref{eqn:nas_linear_const_no_W}) leads to the following optimization problem:

% \begin{equation}
% \label{eqn:nas_linear_const2}
% \begin{array}{l}
% \displaystyle{\min_{\balpha, \bbeta} \mathbb{E}\left[\balpha^T\nabla_{\balpha}\mathcal{L}+\bbeta^T\nabla_{\bbeta}\mathcal{L}\right]}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_i \bbeta_i^s = \sum_k \balpha^s_{k,i}=1}
% \\
% (\balpha^s_{k,i},
% \bbeta^s_i)\in\{0,1\}^2
% \\
% \forall s,k,i.
% \end{array}
% \end{equation}
% \paragraph{FW solver} The above problem can be solved using block coordinate descent on $\balpha, \bbeta$, leading to two problems:


% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_linear_const_alpha}
% \begin{array}{l}
% \displaystyle{\min_{\balpha} \mathbb{E}\left[\balpha^T\nabla_{\balpha}\mathcal{L}\right]}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_k \balpha^s_{k,i}=1} 
% \\
% \balpha^s_{k,i}\in\{0,1\}
% \\
% \forall s,k,i
% \end{array}
% \end{equation}
% \end{minipage}
% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_linear_const_beta}
% \begin{array}{l}
% \displaystyle{\min_{\bbeta} \mathbb{E}\left[\bbeta^T\nabla_{\bbeta}\mathcal{L}\right]}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_i \bbeta^s_{i}=1}
% \\
% \bbeta^s_{i}\in\{0,1\}
% \\
% \forall s,i.
% \end{array}
% \end{equation}
% \end{minipage}

% When $\balpha$ or $\bbeta$ are fixed, problem (\ref{eqn:nas_linear_const2}) is nothing but the expression of a Multiple Choice Knapsack Problem (MCKP) and can be solved either with linear programming or with a greedy algorithm. 
% As for Block-Coordinate Franck-Wolfe, we alternatively solve for $\balpha$ and $\bbeta$ until convergence. This steps requires very few iterations and every iteration solves a MCKP problem with a linear solver that converges in few milliseconds. 
% \paragraph{Initialization} Since FW requires to start from a feasible solution, instead of starting from a random projection in the feasible domain, we seek to start from the most "balanced" initialization, meaning that we want the initial $\balpha, \bbeta$ to be as uniform as possible while respecting the constraints. In order to do so, we solve iteratively the following problems:


% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_init_alpha}
% \begin{array}{l}
% \displaystyle{\min_{\balpha}\sum_{s,k,i}(\balpha^s_{k,i}-\balpha^s_{(k-1),i})^2}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_k \balpha^s_{k,i}=1} 
% \\
% \balpha^s_{k,i}\in\{0,1\}
% \\
% \forall s,k,i
% \end{array}
% \end{equation}
% \end{minipage}
% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_init_beta}
% \begin{array}{l}
%  \displaystyle{\min_{\bbeta}\sum_{s,i}(\bbeta^s_{i}-\bbeta^s_{i-1})^2}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_i \bbeta^s_{i}=1}
% \\
% \bbeta^s_{i}\in\{0,1\}
% \\
% \forall s,i.
% \end{array}
% \end{equation}
% \end{minipage}



% \paragraph{Projection} After the algorithm has converged, the solution might not be binary, due to the update procedure (\ref{eqn:FW_update}). Instead of taking the argmax of every $\balpha,\bbeta$ as done in [TAS] that could lead to an suboptimal solution or violating the time constraint, we solve another linear programming problem with the same constraints as in (\ref{eqn:nas_linear_const_alpha}), (\ref{eqn:nas_linear_const_beta}), and where the objective is replaced with the current $\balpha^k,\bbeta^k$ vectors of the last iteration of the algorithm. 

% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_linear_const_alpha_final}
% \begin{array}{l}
% \displaystyle{\min_{\balpha} \mathbb{E}\left[\balpha^T\balpha^k\right]}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_k \balpha^s_{k,i}=1} 
% \\
% \balpha^s_{k,i}\in\{0,1\}
% \\
% \forall s,k,i
% \end{array}
% \end{equation}
% \end{minipage}
% \begin{minipage}{0.23\textwidth}
% \begin{equation}
% \label{eqn:nas_linear_const_beta_final}
% \begin{array}{l}
% \displaystyle{\min_{\bbeta} \mathbb{E}\left[\bbeta^T\bbeta^{k}\right]}\\
% \text{s.t.} \\
% \balpha^T\Theta\bbeta \leq T
%  \\
% \displaystyle{\sum_i \bbeta^s_{i}=1}
% \\
% \bbeta^s_{i}\in\{0,1\}
% \\
% \forall s,i.
% \end{array}
% \end{equation}
% \end{minipage}



% That way, we are searching for an optimal solution that would be as close as possible as the solution after convergence, and that would respect the constraint. Since this problem is a MCKP problem, we have the the guarantee that the obtained solution is binary.


% The overall algorithm of the procedure is presented in algorithm \ref{alg:BCFW}.

% \begin{algorithm}[tb]
%   \caption{Block-Coordinate Franck-Wolf}
%   \label{alg:BCFW}
% \begin{algorithmic}
% \INPUT Validation set $\mathcal{D}_v$, loss function $\mathcal{L}$
% \FOR{Data batch $x_V$ {\bfseries in} $\mathcal{D}_V$}
% % \FOR{Data batches $(x_T, x_V)$ {\bfseries in} $(\mathcal{D}_T,\mathcal{D}_V)$}

% % \STATE Perform SGD step on weights $W$ using $x_T$.

% \STATE Compute gradients of $\nabla_{\balpha}\mathcal{L}(x_V), \nabla_{\bbeta}\mathcal{L}(x_V)$ .
% \REPEAT 
% \STATE Solve alternatively (\ref{eqn:nas_linear_const2}) for $\balpha$ and $\bbeta$ to find solutions $s_{\balpha}, s_{\bbeta}$ using MCKP solver.
% \UNTIL{convergence}
% \STATE Update $\balpha^{k+1} \leftarrow \balpha^{k}+\gamma(s_{\balpha}-\balpha^{k})$
% \STATE Update $\bbeta^{k+1} \leftarrow \bbeta^{k}+\gamma(s_{\bbeta}-\bbeta^{k})$
% \ENDFOR
% \STATE Solve MCKP problems (\ref{eqn:nas_linear_const_alpha_final}), (\ref{eqn:nas_linear_const_beta_final}) to get optimal solution $\balpha, \bbeta$.
% \OUTPUT $\balpha, \bbeta$

% %   \STATE {\bfseries Input:} data $x_i$, size $m$
% %   \REPEAT
% %   \STATE Compute 
% %   \FOR{$i=1$ {\bfseries to} $m-1$}
% %   \IF{$x_i > x_{i+1}$}
% %   \STATE Swap $x_i$ and $x_{i+1}$
% %   \STATE $noChange = false$
% %   \ENDIF
% %   \ENDFOR
% %   \UNTIL{$noChange$ is $true$}
% \end{algorithmic}
% \end{algorithm}

